The "Giraffe": Discovery of a stripped red giant in an interacting binary with a ${\sim}2~M_\odot$ lower giant

We report the discovery of a stripped giant + lower giant binary, 2M04123153+6738486 (2M0412), identified during a search for non-interacting compact object-star binaries. 2M0412 is an evolved ($T_{\rm eff, giant}\simeq4000$ K), luminous ($L_{\rm giant}\simeq150~L_\odot$) red giant in a circular $P=81.2$ day binary. 2M0412 is a known variable star previously classified as a semi-regular variable. The cross-correlation functions of follow-up Keck/HIRES and LBT/PEPSI spectra show an RV-variable second component with implied mass ratio $q=M_{\rm giant}/M_{\rm comp}\simeq0.20\pm0.01$. The ASAS-SN, ATLAS, TESS and ZTF light curves show that the giant is a Roche lobe filling ellipsoidal variable with an inclination of $49.4^\circ{}\pm{0.3^{\circ}}$, and a giant mass of $M_{\rm giant}=0.38\pm0.01~ M_\odot$ for a distance of $\simeq3.7$ kpc. The mass of the giant indicates that its envelope has been stripped. The giant companion on the lower red giant branch has a mass of $M_{\rm comp}=1.91\pm0.03~M_\odot$ with $T_{\rm eff, comp}\simeq5000$ K, $L_{\rm comp}\simeq60~L_\odot$ and $R_{\rm comp}\simeq11~R_\odot$. We also identify an orbital phase dependent, broad $\rm H\alpha$ emission line which could indicate ongoing accretion from the stripped red giant onto the companion.

==> kochanek_changes.tex <==
estatio $q=0.201\pm0.010$. Theoretical RV curves for mass ratios of $q=0.3$ and $q=0.1$ are shown as red dashed and blue dot-dashed lines respectively. }
    \label{rvsb2}
\end{figure*}

Using just the dynamical information ($K_{\rm giant}$, $K_{\rm comp}$ and $P_{\rm orb}$), we get $a_{\rm orb}\sin i=(a_{\rm giant}+a_{\rm comp})\sin i=80.4\pm0.2~R_\odot$. Using Kepler's third law, this corresponds to $M_{\rm tot}\sin^3 i=(M_{\rm giant}+M_{\rm comp})\sin^3 i=1.06\pm0.01~M_\odot$. Using the constraint on $q$, we can derive the minimum mass of the companion and the giant as
\begin{equation}
    M_{\rm comp}\sin^3 i=0.88\pm0.01~M_\odot,
\end{equation}
and
\begin{equation}
    M_{\rm giant}\sin^3 i=0.18\pm0.01~M_\odot.
\end{equation} For the giant to have the minimum mass given its luminosity, $M_{\rm giant}=M_{\rm core}\simeq0.354~M_\odot$ (Equation \ref{eq:coremass}), $\sin i =0.80\pm0.01$ and $i=53.1\pm1.0^\circ$. At this inclination, $M_{\rm comp}=1.72\pm0.07~M_\odot$, which is again larger than the single star limit from the SED ($M\gtrsim1.4~M_\odot$).

To investigate the second component further, we subtract the best-fit synthetic spectrum of the giant from the HIRES spectra and shift the residuals to the companion's rest-frame. We then calculate the median spectrum from these residuals. As seen in Figure \ref{specsb2}, the median of these residual spectra shows absorption features. If we fit the spectrum with \verb"iSpec" keeping $\rm [M/H]$ fixed at the metallicity of the giant ($\S$\ref{section:giant}), we find $T_{\rm{eff, comp}}=6347\pm700$~K, $\log(g)=3.1\pm0.2$, $\rm [\alpha/Fe]=0.00\pm0.08$, and $v_{\rm rot} \, \textrm{sin} \, i=17.6 \pm 0.6 \, \rm km \,s^{-1}$. As shown in Figure \ref{specsb2}, this model fits the absorption features extremely well. For $i=44^\circ$, $v_{\rm rot} \simeq 25 \, \rm km \,s^{-1}$. A main sequence star with $T_{\rm{eff, comp}}\simeq6400$~K has a mass of ${\sim}1.3~M_\odot$, which is just below the single star SED limit of $M_*\lesssim1.4~M_\odot$. However, a single star with ${\sim}1.3~M_\odot$ cannot account for the mass of the component implied by our constraint on $q$ unless the giant mass is $M_{\rm giant}\simeq0.26~M_\odot$. Additionally, a ${\sim}1.3~M_\odot$ main sequence star cannot exist in a binary with a ${\sim}1.1~M_\odot$ red giant without a history of binary interaction. 

%describe how the second spectrum was derived
\begin{figure*}
	\includegraphics[width=0.9\textwidth]{sb2_lineprofile.pdf}
    \caption{The median spectrum of the second component from 5450~\AA~ to 5550~\AA ~(black) in its rest frame after subtracting the synthetic spectrum of the giant from the HIRES spectra. Model spectra for a star at the giant's metallicity with $T_{\rm eff}=6350$~K and $\log_(g)=3.1$ is shown in blue.}
    \label{specsb2}
\end{figure*}

While making the companion a binary with a compact object would solve this missing mass problem, the radial velocities would then be dominated by the motion of this inner binary and so we would not observe what seems to be the reflex motion of the outer binary. This would be true even for a binary comprised of two stars. For example, an equal mass binary consisting of two $1.3~M_\odot$ stars with a separation $a_{\rm comp}=30~R_\odot$ will have an orbital period of ${\sim}11.8$~days. The velocity of each component in this binary is ${\sim}64\, \rm km \,s^{-1}$ (${\sim}41\, \rm km \,s^{-1}$) for $i=90^\circ$ ($i=40^\circ$), which exceeds the reflex motion (${\sim}8\, \rm km \,s^{-1}$) and the broadening ($v_{\rm rot} \, \textrm{sin} \, i{\sim}18 \, \rm km \,s^{-1}$) observed in the secondary absorption lines. All other configurations of equal mass inner binaries will have shorter orbits and therefore, larger velocities.

To investigate the scenario of a giant + star binary with \verb"PHOEBE", we fit the RVs of the second component along with the RVs of the giant, the ZTF $r$-band + $g$-band light curve, and the \textit{TESS} $T$-band light curve. Instead of a compact object companion, we fit for the radius and temperature of a luminous companion star. We used a prior on the temperature based on the spectral fits ($T_{\rm{eff, comp}}=6347\pm700$~K). For this model, we obtained $M_{\rm giant}=0.626^{+0.054}_{-0.049}~M_\odot$, $M_{\rm comp}=2.72^{+0.18}_{-0.18}~M_\odot$, $R_{\rm giant}=30.8^{+0.9}_{-0.9}~R_\odot$, $R_{\rm comp}=8.8^{+1.2}_{-0.9}~R_\odot$, $T_{\rm{eff, giant}}=4240^{+110}_{-140}$~K, $T_{\rm{eff, comp}}=5950^{+170}_{-290}$~K, $i=44.4^{+1.4}_{-1.1}^\circ$, and $q=M_{\rm giant}/M_{\rm comp}=0.232^{+0.007}_{-0.007}$. This model has $\log(g)=3.0\pm0.1$ for the companion, consistent with the results from fitting the spectra. However, the companion is fairly large and luminous, with $L_{\rm comp}\simeq87~R_\odot$. In the $g$, $r$ and \textit{TESS} bands, the companion contributes ${\sim}43\%$, ${\sim}31\%$ and ${\sim}27\%$ of the total luminosity, respectively. Such a star is inconsistent with the observed SED ($\S$\ref{section:giant}).

Figure \ref{loggteffcomp} shows the position of this companion in $\log(g)$ vs. $T_{\rm eff}$ as compared to a sample of APOGEE DR16 stars. If we search for stars similar to the \verb"PHOEBE" companion in APOGEE DR16, we find 69 stars with $2.5\leq \log(g) \leq 3.5$, ${5600~\rm K}\leq T_{\rm eff} \leq {6400~\rm K}$ and \verb"ASPCAPFLAG"=0. To estimate their radii, we cross-match this list the TESS Input Catalog (TIC) and select 50 sources with radius measurements and distances $<3~\rm kpc$. The $16^{\rm th}$,$50^{\rm th}$ and $84^{\rm th}$ percentile of their radii and luminosity are $R_{\rm *}=4.1^{+2.3}_{-2.5}~R_\odot$ and $L_{\rm *}=16^{+23}_{-14}~L_\odot$.


\begin{figure}
    \vspace{-1cm}
	\includegraphics[width=0.5\textwidth]{loggteff_comp.pdf}
    \vspace{-0.8cm}	
    \caption{$\log(g)$ vs. $T_{\rm eff}$ for the sample of APOGEE DR16 giants. The estimated position of the second component is shown in black.}

    \label{loggteffcomp}
\end{figure}

Another explanation for the second set of absorption lines is that it emerges from an accretion disk surrounding a compact object. In $\S$\ref{section:balmer}, we show that the source has a broad, double-peaked $\rm H\alpha$ emission line in our spectra, and argue that it likely emerges due to an accretion disk. While absorption lines are rarely seen in the spectra of accretion disks, it is not unprecedented. For example, \citet{Strader2016} identified two sets of absorption lines in spectra of the neutron star X-ray binary 3FGL J0427.9$-$6704, which corresponded to the stellar component and the accretion disk. The second set of absorption lines track the reflex motion of the neutron star primary and also matched the velocities derived from the emission features associated with the accretion disk. 

Using \verb"ELC" we tried fitting the ZTF $g$, $r$ and \textit{TESS} light curves along with the radial velocities of the giant and the second component as a star plus a compact object with an accretion disk. We retain the priors from the ELC fits described in $\S$\ref{section:phoebe}, but in this model we keep the temperature of the giant fixed at $T_{\rm eff, giant}=4150$~K. For the disk, we fit the inner $r_{\rm in}$ and outer radii $r_{\rm out}$ in units of the Roche radius of the compact object $r_{\rm RL}$, the temperature $T_{\rm in}$ of the disk at $r_{\rm in}$, the power-law exponent on the temperature profile of the disk $T(r)\propto T_{\rm in}(r/r_{\rm in})^{\xi}$, and the opening angle of the disk rim above the plane $\beta$. We find $M_{\rm giant}=0.72^{+0.04}_{-0.03}~M_\odot$, $M_{\rm comp}=3.11^{+0.11}_{-0.08}~M_\odot$, $R_{\rm giant}=32.2^{+0.6}_{-0.5}~R_\odot$, $i=42.4^{+0.5}_{-0.6}^\circ$, and $q=M_{\rm giant}/M_{\rm comp}=0.184^{+0.041}_{-0.079}$. For the disk, we obtain $r_{\rm in}/r_{\rm RL}=0.020^{+0.019}_{-0.014}$, $r_{\rm out}/r_{\rm RL}=0.819^{+0.126}_{-0.135}$, $T_{\rm in}=9000^{+7100}_{-1600}$~K, $\xi=-0.52^{+0.06}_{-0.12}$, and $\beta=30.3^{+15.0}_{-23.6}^\circ$. This model is, however, a slightly significantly worse fit than the \verb"ELC" models without any emission from the companion. In physical units the disk spans from $r_{\rm in}\simeq1.3~R_\odot$ to $r_{\rm out}\simeq51.4~R_\odot$ compared to a Roche limit for the secondary of $r_{\rm RL}\simeq62.8~R_\odot$. While the origin of absorption lines from a disk remains an issue, the temperatures of the disk in the inner regions of this model are not in gross conflict with the model of the spectrum.

The presence of the secondary RV component raises an interesting dilemma. Given the expected mass of the giant from our \verb"PHOEBE" model in $\S$\ref{section:phoebe} ($M_{\rm giant}\simeq0.6~M_\odot$), the mass ratio required by the radial velocities require $M_{\rm comp}\simeq3.0~M_\odot$, entirely consistent with the estimate from \verb"PHOEBE". However, a stellar companion with this mass would be trivially visible in the SED (Figure \ref{sedfit}), especially towards the UV. For example, a ${\sim}3.0~M_\odot$ main sequence B star with a temperature of ${\sim}11,000$~K and a luminosity ${\sim}100~L\odot$ can be easily ruled out.

\clearpage
\clearpage

\subsection{Balmer $\rm H\alpha$ emission} \label{section:balmer}

As shown in Figure \ref{spechalpha}, there is a broad $\rm H\alpha$ emission line whose structure varies with the orbital phase. V723 Mon also has this property \citep{Jayasinghe2021}, but here it is directly visible without any need to subtract the stellar spectrum.

We identify both blue-shifted and red-shifted emission components in most of our spectra. We define these components by the wavelength ranges of $6560-6562~\angstrom$ and $6564-6566~\angstrom$ respectively. The most significant $\rm H\alpha$ emission in our spectra is seen near phase $\phi{\sim}0.9$ as a blue-shifted component. The emission component has a velocity close to the rest frame of the giant near phase $\phi{\sim}0.25$ and fills in the giant's $\rm H\alpha$ absorption line. Near phase ${\sim}0.9$, the typical Gaussian FWHM of the blue-shifted (red-shifted) $\rm H\alpha$ emission component is ${\sim}255\, \rm km\,s^{-1}$ (${\sim}265\, \rm km\,s^{-1}$). The wings of the emission extends beyond ${\sim}200\, \rm km\,s^{-1}$ in some of our spectra. 

The peak separations at $\phi{\sim}0.1$ and $\phi{\sim}0.9$ are ${\sim}160\, \rm km\,s^{-1}$ and ${\sim}196\, \rm km\,s^{-1}$ respectively. However, the behavior of the double-peaked profile appears to vary between orbits. For example, we obtained Keck/HIRES spectra near $\phi{\sim}0.1$ in two consecutive orbits, where the first spectrum has a peak separation of ${\sim}106\, \rm km\,s^{-1}$ and the second spectrum has a much larger peak separation of ${\sim}160\, \rm km\,s^{-1}$. For the epochs where we can see a double-peaked emission profile, the median peak separation is ${\sim}168\, \rm km\,s^{-1}$ with a scatter of $\sigma{\sim}31\, \rm km\,s^{-1}$. The orbital phase evolution and profile morphology of the $\rm H\alpha$ emission is qualitatively similar to that seen in the red giant + neutron star binary 1FGL J1417.7$-$4407 \citep{Strader2015}.

Figure \ref{orbhalpha} shows the $\rm H\alpha$ line at various orbital phases along with the  \verb"PHOEBE" models of the orbital configurations of the binary. After conjunction at $\phi\simeq0.5$, the emission is blue-shifted and reaches a maximum at phase $\phi{\sim}0/1$ (Figure \ref{ewphase}). Since the $\rm H\alpha$ emission varies significantly in the rest-frame of the giant, this emission must emerge from beyond the giant's photosphere. Given its large FWHM, we can rule out a chromospheric origin for the $\rm H\alpha$ emission. We do not observe the $\ion {Ca}{ii}$ H and K emission lines that are typically associated with chromospheric activity,

Figure \ref{halphasub} shows the $\rm H\alpha$ line profiles after subtracting the template spectrum of the red giant. We see a blue-shifted $\rm H\alpha$ absorption feature in these line profiles at a roughly constant ${\sim}30\, \rm km\,s^{-1}$ blue shift relative to the giant. The depth of the absorption core is strongest near $\phi{\sim}0.5$. The velocity of this absorption feature is close to the velocity of the giant's photosphere ($v_{\rm rot, giant}\simeq 20\, \rm km\,s^{-1}$), consistent with mass outflow from the giant at $L_1$. At $\phi=0$, the inner Lagrangian point ($L_1$) is directed toward the observer and at $\phi=0.5$, $L_1$ points away from the observer \citep{Beech1985}. It is possible that the absorption feature is associated with density enhancements caused by matter streaming through the inner Lagrangian point. 

Figure \ref{ewphase} shows how the equivalent width varies with orbital phase for both the blue-shifted and red-shifted $\rm H\alpha$ components. The largest equivalent width of the blue-shifted (red-shifted) $\rm H\alpha$ component is $\rm EW(H\alpha){\sim}-0.5$ ($\rm EW(H\alpha){\sim}-0.3$) at $\phi{\sim}0.9$. These equivalent widths are more than an order of magnitude smaller than those observed for X-ray binaries (see, for e.g., \citealt{Fender2009}) and correspond to a total line luminosity of ${\sim}0.003~L_\odot$. For both the blue and red components, the equivalent widths are the most negative (emission is strongest) near $\phi{\sim}0$ when the companion is on the near side of the giant. The red-shifted line also has a weaker peak at $\phi{\sim}0.5$ when the companion is on the far side. We are unable to do a similar analysis for the $\rm H\beta$ line because it is not included in the HIRES spectra and the PEPSI S/N is poor at $\rm H\beta$. 

If we interpret the double peaked structure as an accretion disk, the projected radial velocity of the outer rim of an accretion disk is approximately equivalent to half the velocity separation of the two peaks $V_h$ (see, for e.g., \citealt{Smak1981,Strader2015}). In this case, the $V_h$ of $84\, \rm km\,s^{-1}$ is significantly larger than the radial velocity semi-amplitude of the red giant (${\sim}42\, \rm km\,s^{-1}$). It is also slightly larger than the circular velocity at the surface of the giant (${\sim}78\, \rm km\,s^{-1}$ for $M=1~M_\odot$ and $R=31~R_\odot$). Indeed, $V_h$ is expected to be larger than the radial velocity semi-amplitude of the giant for classical Keplerian disks (see, for e.g., \citealt{Paczynski1977,Orosz1994}). As an orbit around the secondary, this velocity corresponds to ${\simeq}27~M_{\rm comp}\sin^2i ~R_\odot$ or ${\simeq}11~M_{\rm comp} ~R_\odot$ if we use a disk inclination of $40^\circ$.

In summary, we observe a phase dependent, broad ($\gtrsim200\, \rm km\,s^{-1}$)  $\rm H\alpha$ emission line in our spectra of 2M0412. We show that the morphology and orbital evolution of the $\rm H\alpha$ emission is likely due to an accretion disk. This is consistent with our interpretation of this system where the red giant nearly fills its Roche lobe. However, more spectra are needed to study the behavior of the $\rm H\alpha$ emission in better detail.

\begin{figure}
    
    \includegraphics[width=0.5\textwidth]{halpha_lineprofiles.pdf}
    \caption{$\rm H\alpha$ line profiles in the rest frame of the giant in the HIRES and PEPSI spectra. The line profiles are sorted and colored as a function of orbital phase.}
    \label{spechalpha}
\end{figure}

\begin{figure}
	\includegraphics[width=0.5\textwidth]{halpha_orbit.pdf}
	
    \caption{Behavior of the $\rm H\alpha$ line profiles with orbital phase. The right panels show the $\rm H\alpha$ line profiles at the orbital configurations illustrated in the left panels. The size of the companion is simply chosen to make it easily visible. The red dashed line shows the best fit synthetic spectrum for the giant.}
    \label{orbhalpha}
\end{figure}

\begin{figure*}
	\includegraphics[width=\textwidth]{halpha_giantsub.pdf}
	
    \caption{Variations of the $\rm H\alpha$ line profiles with orbital phase in the giant's rest frame after subtracting a template spectrum for the red giant. The left panel shows the full wavelength range and the right panel zooms in on the line core. Note the $\rm H\alpha$ absorption feature at ${\simeq}-30\, \rm km\,s^{-1}$ in the giant's rest-frame.}
    \label{halphasub}
\end{figure*}

\begin{figure*}
    
    \includegraphics[width=1\textwidth]{ew_phase.pdf}
    \caption{Equivalent width of the blue-shifted (blue points, $6560-6562~\angstrom$) and red-shifted (red points, $6564-6566~\angstrom$) $\rm H\alpha$ emission components as a function of orbital phase.}
    \label{ewphase}
\end{figure*}

\subsection{X-ray upper limit} \label{section:xrays}

No X-rays were detected in the \textit{Swift} XRT observations. We derived a 3 sigma upperlimit using the reprocessed observations of sw00014417001 (${\sim}2.2$~ks), a 50 arcsec source region centered on the source and a 150 arcsec source free background region located at $(\alpha_{J2000}, \delta_{J2000})$=(04:12:38.10,67:43:00.86). We derive an aperture corrected 3$\sigma$ upper limit on the 0.3-2.0 keV count rate of $8.1\times10^{-4}$ counts/s. Using the Galactic column density along the line of sight ($N_{H}\sim1.34\times10^{22}$ cm$^{-2}$, \citealt{HI4PICollaboration2016}), and an absorbed power-law with a photon index of 2, we derive an absorbed (unabsorbed) flux of $1.7\times10^{-14}$ erg cm$^{-2}$ s$^{-1}$ ($5.0\times10^{-14}$ erg cm$^{-2}$ s$^{-1}$), which corresponds to an absorbed (unabsorbed) X-ray luminosity of $3.4\times10^{31}$ erg s$^{-1}$ ($9.5\times10^{31}$ erg s$^{-1}$). The \textit{Swift} XRT upper limit is compatible with the X-ray luminosities expected of quiescent X-ray binaries ($L_{\rm X}\sim10^{30}-10^{31}~ \rm ergs~s^{-1}$; \citealt{Dincer2018}). If the X-ray luminosity originates from an accretion disk around a ${\sim}3.0~M_\odot$ black hole, the luminosity is ${\lesssim}1.1\times10^{-7}~L_{\rm edd}$. 

We estimate the mass loss rate from the giant as
\begin{equation}
    \dot{M}=4\times10^{-13}~\eta_R ~\frac{LR}{M}\,M_\odot {\rm yr^{-1}} \approx 2\times10^{-9} \,M_\odot {\rm yr^{-1}},
\end{equation} \citep{Reimers1975} where $L$, $R$ and $M$ are in solar units and $\eta_R\simeq0.477$ \citep{McDonald2015}. The velocity of the wind from the giant is assumed to be the escape velocity, $V_{\rm wind}\approx V_{\rm esc}\sim90\rm \,km~s^{-1}$. For a scenario with wind-fed accretion to the compact object, \citet{Thompson2019} approximated the amount of material gathered at the sphere of influence of the black hole as \begin{equation}
\begin{aligned}
& \dot{M}_{\rm acc}\sim \frac{\pi \dot{M}}{(4\pi a_{\rm giant}^2)}\, \left(\frac{G M_{\rm BH}}{V_{\rm wind}^2}\right)^2\\
& \sim7\times10^{-11}\,{\rm M_\odot\,\,yr^{-1}}\,\,\, \dot{M}_{-9}\bigg(\frac{M_{\rm BH}}{3 M_\odot}\bigg)^2 \bigg(\frac{V_{\rm wind}}{120 \rm \,km~s^{-1}}\bigg)^{-4}\\
& \sim 4\times10^{-10}\,{\rm M_\odot\,\,yr^{-1}},
\end{aligned}
\end{equation} where $\dot{M}_{-9}=\dot{M}/10^{-9}$\,M$_\odot$ yr$^{-1}$. For radiatively efficient accretion, the luminosity would be
\begin{equation}
    L_{\rm acc}\sim0.1~\dot{M}_{\rm acc}~c^2\simeq630~L_\odot\simeq 7\times 10^{-3}~L_{\rm Edd}.
\end{equation}
This estimate of the accretion luminosity is much larger than the observed X-ray luminosity of this system (${\lesssim}0.01~L_\odot$) but for radiatively inefficient accretion, the luminosity can be much lower \citep{Narayan1995}.

\clearpage
\clearpage

\section{The Nature of the Companion}

\label{section:darkcomp}

In this section, we systematically discuss the nature of the companion given the observed properties of the system and the modeling results from $\S$\ref{section:results}. Figure \ref{masses} summarizes the overall landscape of the constraints on the masses of the giant and the companion. In all scenarios, the models have mass ratios $q=0.2$ to $0.3$ and inclinations of $i=30^\circ$ to $50^\circ$.The various \verb"ELC" and \verb"PHOEBE" models are marked. That the companion RV signal corresponds to a simple reflex motion of the giant and the associated absorption features are narrow rules out making the companion a binary containing a star, so we focus on a system where the companion is a single star. If the companion is a single star without any binary interactions, its maximum mass is $1.7M_\odot$ and this requires a companion just evolving off the main sequence onto the sub-giant branch. If it is still on the main sequence it must be less massive than $1.4M_\odot$, and this limit is shown in Figure~\ref{sedfit} and \ref{masses}.

Assuming the inclination and mass ratio are well-constrained, the only way to have a low mass companion is for the single-star evolution estimates of the mass of the giant ($\S$\ref{section:giant}) to be wrong as a result of recent binary stellar mass transfer and interaction. In such a scenario, the observed giant was initially more massive, but has recently lost mass to the companion, and single-star evolutionary models based on the luminosity and temperature then lead to an overestimate of the present day giant mass. Additionally, the companion that has gained mass needs to be much less luminous than a star with its present-day mass.

There are, however, several constraints on the giant mass that are independent of single star evolution models. First, the giant is on the upper RGB and not on the red clump (Figure \ref{loggteff}), so it has a degenerate core. The luminosity of a giant with a degenerate core of mass $M_{\rm core}$ is
\begin{equation}
    \label{eq:coremass}
    \bigg(\frac{L}{L_\odot}\bigg)\approx 675 \bigg(\frac{M_{\rm core}}{0.4~M_\odot}\bigg)^{7}.
\end{equation} \citep{Boothroyd1988}, so we must have $M_{\rm giant}>M_{\rm core}\simeq0.34~M_\odot$ for $L\sim230~L_\odot$. Second, the giant must lie inside its Roche limit. Using the \citet{Eggleton1983} approximation for the Roche limit, we see in Fig.~\ref{masses} that the giant must be more massive than $M_{\rm giant} \gtorder 0.5~M_\odot$ for the radius of $R{\simeq}29~R_\odot$ from the SED ($\S$\ref{section:giant}). Note that this limit is identical to the argument that the mean density of a Roche lobe filling star is largely determined by the period (\citealt{Eggleton1983}) which was used by \cite{El-Badry2021} in arguing against the NGC~1850 BH1 candidate discussed in the introduction. If the star is tidally locked, it cannot fully fill its Roche lobe (i.e. the Roche radius cannot be made consistent with the stellar radius needed for locking), so the star must lie to the right of these limits and not lie exactly on them. Thus, if the giant is at least as large as $29 ~R_\odot$, the companion must have $M_{\rm comp} \gtorder 1.7 ~M_\odot$ if $q<0.3$ or $i < 50^\circ$.


\begin{figure*}
        \vspace{-1cm}
    \includegraphics[width=\textwidth]{massplot.png}
        \vspace{-0.7cm}
    \caption{The mass of the companion ($M_{\rm comp}$) as a function of the mass of the giant ($M_{\rm giant}$). The binary mass function at inclinations of $i=90^\circ$, $40^\circ$ and $30^\circ$ are shown as the blue dashed lines. Giants with radii of $R=25~R_\odot$, $R=29~R_\odot$ or $R=33~R_\odot$ will overfill their Roche lobes if they have masses less than the Roche limits given by the dashed curves. The companion masses for a mass ratio of $q=0.2$ and $q=0.3$ are shown as the red lines. The orange shaded region highlights giant masses that are not allowed by the condition $M_{\rm giant}\gtrsim M_{\rm core}\simeq0.34~M_\odot$ (Equation \ref{eq:coremass}). The green shaded region shows companion masses for luminous stars that are allowed by the single star SED limit ($M_*\lesssim1.4~M_\odot$, $\S$\ref{section:giant}, Figure \ref{sedfit}). The derived values for $M_{\rm comp}$ and $M_{\rm giant}$ from the PHOEBE models at fixed giant radii ($\S$\ref{section:phoebe}, Table \ref{tab:phoebefitsrfixed}) are shown in black.}
    \label{masses}
\end{figure*}

Evading this limit requires making the star physically smaller. It does not seem feasible to do this by raising the temperature. The SED models and the models of the spectra are in excellent agreement on the temperature of the giant. If the temperature is known, the only way to reduce the stellar radius is to reduce the distance since for fixed temperature, $R_{\rm giant} \propto L_{\rm giant}^{1/2} \propto d$. We have been using a distance of $d =4.0$~kpc based on the parallax corrected for the global zero-point parallax offset in \textit{Gaia} EDR3. \citet{Bailer-Jones2021} find a distance of $d=3.7$~kpc, which is almost 8\% smaller. The distance derived using the zero-point offset corrections from \citet{Lindegren2021}, while consistent with the \citet{Bailer-Jones2021} distance, might be biased due to an over-correction of the zero-point parallax offset (see, for e.g., \citealt{Groenewegen2021,Bhardwaj2021,Zinn2021}). Alternatively, \citet{Hogg2019} find a distance of $d=4.4$~kpc using a spectrophotometric parallax, which is 10\% larger. A smaller distance would reduce the radius to $R_{\rm giant}=27~ R_\odot$ and the Roche limit would allow the giant to have a mass as low as $M_{\rm giant} \gtorder 0.4~M_\odot$. The \citet{Bailer-Jones2021} method, however, uses a prior that weights distances based on the expected numbers of stars without reference to the stellar type. Since giants have larger distances than dwarfs at fixed magnitude, a prior based on all stars will generally bias the distance estimates to a giant to be low. Reducing the distance also tightens the SED limits on any companion: in Figure \ref{sedfit}, the SED of the giant moves downwards while the SEDs of possible companions are unchanged. 

Assuming tidal synchronization, we can also use $v_{\rm rot}\sin i$ to estimate the radius of the giant
\begin{equation}
      R\sin i= 19.3 ~ R_\odot \bigg(\frac{v_{\rm rot}\sin i}{12\, \rm km \,s^{-1}}\bigg),
\end{equation} which gives $R_{\rm giant}=38.5~R_\odot$, $29.9~R_\odot$, $25.1~R_\odot$, and $22.2~R_\odot$ for $i=30^\circ$, $40^\circ$, $50^\circ$, and $60^\circ$. \verb"isoclassify" single star evolution models based on the spectroscopic parameters and the photometry used in the SED model given an estimated mass of $M_{\rm giant} = 1.11_{-0.22}^{+0.24}~M_\odot$ and a radius of $R_{\rm giant}=29.8^{+2.2}_{-2.0}~R_\odot$. The spectroscopic $\log g$ estimates give a mass of $M_{\rm giant} = 0.9 \pm 0.6 M_\odot$ that is consistent with any of these estimates.  

\subsection{Comparison to BPASS binary evolution models} \label{section:bpass}

As an initial experiment we used \verb"hoki" \citep{Stevance2020} to search for Binary Population And Spectral Synthesis (BPASS; \citealt{Eldridge2017,Stanway2018}) binary models consistent with the observed properties of 2M0412. We used the BPASS v2.2.1 models at $\rm Z=0.006$, which is the closest match to the metallicity derived in $\S$\ref{section:giant}. 

We restrict our search to models with
\begin{enumerate}
  \item Period of the binary, $P_{\rm orb}=81\pm8$~days,
  \item $V=-0.61\pm1$~mag,
  \item $J=-2.87\pm1$~mag,
  \item $K=-3.68\pm1$~mag,
  \item Total luminosity of the binary, $ \log(L_{\rm binary})=2.40\pm0.05$, 
  \item Radius of the giant, $ \log(R_{\rm giant})=1.49\pm0.05$, 
  \item Effective temperature of the giant, $\log(T_{\rm eff})=3.62\pm0.05$, 
  \item Mass of the giant, $M_{\rm giant}=[0.35,2]~M_\odot$, and
  \item Binary mass ratio, $0.15<q<0.35$.
\end{enumerate}

We searched for models where either (1) the companion is a star with an effective temperature lower than $T_{\rm eff, comp}<7000$~K, or (2) the companion is a compact object. We found 11 giant + star and 19 giant + compact object models that satisfied these criteria. In all of the models, the giant 
is heavily stripped with masses in the range of ${\sim}0.38-0.60~M_\odot$ ($M_{\rm init}\simeq1.4-2.3~M_\odot$) and ${\sim}0.36-0.79~M_\odot$ ($M_{\rm init}\simeq0.9-2.5~M_\odot$) for the giant + star and the giant + compact object models, respectively. Table \ref{tab:bpass} gives the models closest in period and magnitude ($P_{\rm orb}=81\pm2$~days, $\Delta(M)=0.5$~mag) as examples.

The BPASS model that best matches our observations and derived properties is a giant + compact object binary. In this model, $M_{\rm giant}\simeq0.78~M_\odot$, $M_{\rm comp}\simeq3.71~M_\odot$, $q\simeq0.21$, $R_{\rm giant}\simeq30.6~R_\odot$, $T_{\rm eff, giant}\simeq4246~\rm K$, $\Delta(V)=0.09$~mag, $\Delta(J)=0.04$~mag, and $\Delta(K)=0.01$~mag. Given that Roche lobe overflow (RLOF) has now ceased, this binary will have a similar orbital configuration (period and semi-major axis) for ${\sim}173$~Myr. Over a period of ${\sim}2$~Myr, the giant lost ${\sim}69\%$ of its pre-RLOF mass through RLOF. The three other giant + compact object binary models in Table \ref{tab:bpass} are still undergoing RLOF with total durations of ${\sim}5-21$~Myr. Unlike the best match model, the other binaries are on rapidly evolving configurations as RLOF is still ongoing. In these three models, the giant ultimately loses ${\sim}57-77\%$ of its initial mass.

The giant + star binary that best matches our data has $M_{\rm giant}\simeq0.60~M_\odot$, $M_{\rm comp}\simeq2.15~M_\odot$, $q\simeq0.280$, $R_{\rm giant}\simeq33.5~R_\odot$, $T_{\rm eff, giant}\simeq4039~\rm K$, $\Delta(V)=0.06$~mag, $\Delta(J)=0.01$~mag, and $\Delta(K)=0.14$~mag. Comparing this model with the best giant + compact object model, the current configuration of the giant + star binary is short-lived, with the orbit expanding to a period of ${\sim}102$~days in ${\sim}1.4$~Myr. In this model, the binary is undergoing RLOF with a total duration of ${\sim}13$~Myr. The two other giant + star binary models in Table \ref{tab:bpass} have similar properties. In these models, the giant loses ${\sim}63-69\%$ of its initial mass. For a conservative mass-transfer binary, the accretor is spun up and will therefore be rapidly rotating. The companion star to the giant is ${\sim}2.9-3.4$~mag ($F_{\rm comp}/F_{ \rm binary}{\sim}4.2\%-6.7\%$) and ${\sim}3.6-4.1$~mag ($F_{\rm comp}/F_{ \rm binary}{\sim}2.4\%-3.6\%$) fainter than the overall binary in the $V$ and $R$ bands, respectively. Based on the NUV limits, we only can only very weakly rule out such companions. 

%Figure \ref{sedbpass} shows the SEDs of the companion stars in these BPASS models along with the observed SED of 2M0412. 

\begin{table*}
	\centering
	\caption{Properties of the BPASS models that match observations for 2M0412.}

\begin{threeparttable}	
\begin{tabular}{rrrrrrrrrrrrrrr}
		\hline
		\vspace{1mm}	
		 Model & $M_{\rm giant}$ & $M_{\rm He~core}$ & $M_{\rm comp}$ & $q$ & $T_{\rm eff, giant}$ & $T_{\rm eff, comp}$ & $R_{\rm giant}$ & $R_{\rm comp}$  & $L_{\rm giant}$ & $P_{\rm orb}$ & Age\\
		  & $(M_{\odot})$ & $(M_{\odot})$ & $(M_{\odot})$ & & $(\rm K)$ & $(\rm K)$ & $(R_{\odot})$ & $(R_{\odot})$ & $(L_{\odot})$ &  $(\rm d)$ &  Gyr\\		 
		\hline
        1 & 0.49 & 0.33 & 1.70 & 0.288 & 4036 & 6860 & 31.0 & 1.5 & 230  & 83.0 & 1.8 \\
        2 &0.52 & 0.32 & 1.81 & 0.289 & 4034 & 6273 & 31.0 & 1.9 & 229  & 80.4 & 2.7\\
        3 & $^{\rm a}~$0.60 & 0.33 & 2.15 & 0.280 & 4039 & 6871 & 33.5 & 2.1 & 269 & 83.1 & 1.8\\        
		\hline
        4& 0.48 & 0.32 & 3.02 & 0.160 & 4073 & -- & 31.3 & -- & 243 & 82.3 & 0.8 \\
        5 & 0.51 & 0.32 & 2.39 & 0.214 & 4044 & -- & 30.7 & -- & 226  & 80.8 & 2.1 \\
        6& 0.60 & 0.32 & 2.19 & 0.276 & 4045 & -- & 32.8 & -- & 259 & 80.9 & 2.6 \\	
        7& $^{\rm b,~c~}$0.78 & 0.38 & 3.71 & 0.210 & 4246 & -- & 30.6 & --& 278 & 81.1 & 0.5\\            
		\hline        
\end{tabular}
    \begin{tablenotes}
      \small
      \item $^{\rm a}$ Best matching giant + star model.
      \item $^{\rm b}$ Best matching giant + compact object model.   
      \item $^{\rm c}$ Best overall model.      
    \end{tablenotes}

\end{threeparttable}
\label{tab:bpass}
\end{table*}


\begin{table*}
	\centering
	\caption{Properties of the MESA binary models for the giant + star binaries in BPASS that match observations for 2M0412. The initial masses of the stars are listed as $M_1$ and $M_2$. The MESA binaries are evolved from an initial orbital period of 25.2~days.}

\begin{threeparttable}	
\begin{tabular}{rrrrrrrrrrrrrr}
		\hline
		\vspace{1mm}	
		 Model & $M_{1}$  & $M_{2}$ & $M_{\rm giant}$  & $M_{\rm comp}$ & $q$ & $T_{\rm eff, giant}$ & $T_{\rm eff, comp}$ & $R_{\rm giant}$ & $R_{\rm comp}$  & $L_{\rm giant}$ & $L_{\rm comp}$ & $P_{\rm orb}$ & Age\\
		 
		  & $(M_{\odot})$ & $(M_{\odot})$ & $(M_{\odot})$ & $(M_{\odot})$ & & (K) & (K) & $(R_{\odot})$ & $(R_{\odot})$ & $(L_{\odot})$ & $(L_{\odot})$ &  $(\rm d)$ &  Gyr\\		 
		\hline
        1 & 1.60 & 1.28 &0.61 & 2.27 & 0.270 & 4096 & 11692 & 29.4 & 1.6 & 220 & 43  & 81.10 & 1.7\\
        2 & 1.40 & 1.26 & 0.57& 2.09 & 0.274 & 4094 & 10780 & 28.7 & 1.7 & 209 & 35 & 81.16 & 2.6\\         
        3 & 1.60 & 1.44 & 0.65 & 2.39 & 0.274 & 4103 & 11730 & 30.2 & 1.8 & 232 & 57  & 81.12 & 1.7\\
		\hline
\end{tabular}


\end{threeparttable}
\label{tab:mesa}
\end{table*}

We were puzzled by (in particular) the low temperatures of the stellar companions in the BPASS models. The cause is that the present BPASS models only evolve one star at a time for reasons of speed \citep{Eldridge2016}. This can lead to misestimates of the properties of the accreting star (Eldridge, private comm.). To examine this, we evolved the BPASS giant + star binaries (Models 1-3, Table \ref{tab:bpass}) using Modules for Experiments in Stellar Astrophysics \citep[MESA][]{Paxton2011, Paxton2013, Paxton2015, Paxton2018, Paxton2019}. MESA computes Roche lobe radii in binary systems using the fit of \citet{Eggleton1983}, and the mass transfer rates in Roche lobe overflowing binary systems are determined following the prescription of \citet{Kolb1990}. We adopt the explicit mass transfer calculation scheme in MESA. We use the initial component masses and orbital period ($P_{\rm orb,init}=25.2$~days) from the BPASS models and examine their properties when the binary has a period of $P_{\rm orb}{\sim}81$~days. As in the BPASS models, the initially more massive component becomes a red giant with $M_{\rm giant}\simeq0.57-0.65~M_\odot$ and its companion is a main sequence star with $M_{\rm comp}\simeq2.09-2.39~M_\odot$. The giant's properties of $T_{\rm eff, giant}\simeq4094-4103$~K, $R_{\rm giant}\simeq28.7-30.2~R_\odot$, $\log(g)\simeq1.3$ and $L_{\rm giant}\simeq209-232~L_\odot$ are virtually identical to those of the observed stars. For all three models, the giant is still in the process of transferring mass to its companion when it reaches this period. Once the mass transfer is complete, the binary is at an orbital period of $P_{\rm orb}\simeq220-281$~days.

In the MESA models, however, the companion to the giant is a hot, luminous star with $T_{\rm eff, comp}\simeq10800-11700$~K, $R_{\rm comp}\simeq1.6-1.8~R_\odot$, $\log(g)\simeq4.3$ and $L_{\rm comp}\simeq35-57~L_\odot$. Such a hot companion is grossly incompatible with the NUV limits from \textit{Swift} and \textit{GALEX} ($\S$\ref{section:giant}, Figure \ref{sedfit}). This is also significantly hotter than the temperature derived for the second component from fitting the spectra ($T_{\rm{eff, comp}}=6347\pm700$~K) or the two star \verb"PHOEBE" models ($T_{\rm{eff, comp}}=5950^{+170}_{-290}$~K). The key points are that the higher temperatures in the {\tt MESA} models are more consistent with the companion mass and evolutionary state and would also make the companion easily visible.  

\subsection{Discussion}

Table~\ref{tab:scenarios} summarizes all of the possible system configurations with single or binary companions comprised of stars, white dwarfs, neutron stars or black holes. We think all binary companions including a star are ruled out by the effect of the orbital motion of the star in the inner binary on the apparent velocity and absorption lines that seem to be associated with the companion. A single WD would be above the Chandrasekhar limit. A single neutron star is also ruled out unless the giant mass can be driven as low as $M_{\rm giant}=0.45~M_\odot$ to allow a $<2.3~M_\odot$ neutron star \citep{Raaijmakers2020}. Another problem for either a WD or a NS is that there is likely some accretion and it is not possible for accretion onto these systems to be radiatively inefficient because they have surfaces. A low mass black hole is plausible if the giant's mass is $M_{\rm giant} \gtorder 0.6 M_\odot$ so that it can be $\gtorder 3M_\odot$. A black hole also allows for accretion with little radiation because the accretion energy can be advected into the black hole rather than being radiated.

Given the luminosity of the giant, single star evolutionary models require high enough masses for the giant, $M_{\rm giant} \simeq 1 M_\odot$ that there is little option other than making a single companion a black hole. However, if the companion is stellar, this is almost certainly a mass transfer system where the giant has lost mass to the companion and so is less massive than predicted by single star models of its luminosity and temperature. A key problem is that ellipsoidal variability really only depends on ratios -- mass ratios and radius/semi-major axis ratios -- so the mass scale requires an estimate of the mass of the giant. For our previous system V723 Mon \citep{Jayasinghe2021}, the velocity residuals analyzed by \citet{Masuda2021} break any degeneracy because they provide a constraint on the strength of the ellipsoidal variability with units. If the radius of the giant can be made small enough to allow a low mass giant ($M_{\rm giant}\ltorder 0.5~M_\odot$) and the accreting companion can be as low temperature as in the BPASS (but not the MESA) models, then it is possible for the companion to be a star. In $\S$\ref{section:phoebe}, we fit \verb"PHOEBE" models to the ZTF $r$-band and \textit{TESS} light curves at fixed radii. Even at a radius of $R=23~R_\odot$ (which implies a distance of $d\simeq3.2$~kpc), the mass of the companion is $M_{\rm comp}\simeq2.1~M_\odot$. For a stellar companion to remain undetected in the SED, the mass ratio has to be $q>0.3$, which is inconsistent with all of the \verb"PHOEBE" models in $\S$\ref{section:phoebe} and the dynamical measurement from $\S$\ref{section:ccf}.

For completeness, Table~\ref{tab:scenarios} also summarizes the possible double compact object binary companions. A double WD binary can be ruled out because each WD will have a mass that is very close to or exceeds the Chandrasekhar limit. Combining a WD and a NS is allowed, and the NS mass is in the observed range if the WD mass is $>0.9~M_\odot$.A double NS binary is feasible. They would need to be of similar mass, since a mass ratio $>0.67$ is needed to keep the lower mass NS above the theoretical minimum of $1.2~ M_\odot$ \citep{Suwa2018}.  BH plus NS or WD binaries are unlikely as they drive the BH mass further into neutron star territory. A double BH binary seem implausible because they both require BH masses in the range observed for neutron stars. The simplest explanation is again that the dark companion is a mass gap black hole or a high mass neutron star.

Figure \ref{masscomp} shows the masses of black holes discovered through electromagnetic methods, including X-ray binaries and non-interacting systems, as a function of their orbital period. The BH masses and orbital periods of the X-ray binaries are from \citet{Tetarenko2016}. The masses of the non-interacting BHs in the field appear to be lower than expected when compared to the BH mass distribution of the X-ray binaries. A larger sample of non-interacting BHs will be useful to study this mass distribution further.

\begin{figure*}
    \vspace{-1cm}    
    \includegraphics[width=1.05\textwidth]{masslogplogm.png}
    \vspace{-0.5cm}    
    \caption{BH masses as a function of orbital period for X-ray binaries (black), non-interacting binaries in globular clusters (blue; \citealt{Giesers2018,Giesers2019}) and non-interacting binaries in the field (red; \citealt{Thompson2019,Jayasinghe2021}). The BH masses and periods for the X-ray binaries are from \citet{Tetarenko2016}. From the limited sample of non-interacting compact objects in the field, we see hints that the typical non-interacting BH masses are lower than expected from the mass distribution of the X-ray binaries.}

    \label{masscomp}
\end{figure*}


\begin{table*}
	\centering
	\caption{Comparison of the possible scenarios involving stellar companions (*), white dwarfs (WD), neutron stars (NS) and black holes (BH) that can explain the nature of the companion. We assumed $M_{\rm comp}\simeq3.0~M_\odot$ from the PHOEBE model with $R_{\rm giant}=29~R_\odot$ ($\S$\ref{section:phoebe}, Table \ref{tab:phoebefitsrfixed}). A `\cmark' indicates that the scenario is possible, a `?' indicates that while the scenario is technically possible, it is very unlikely and a `\xmark' indicates that the scenario is ruled out. The simplest explanation is that of a single low mass black hole, indicated with `\cmark \cmark'.}
\begin{threeparttable}	
\begin{tabular}{rrr}
		\hline
		 Dark Companion & Possibility & Comment \\
		 \hline
		 \vspace{1mm}		 
		 Single Star & ? & Hot, main sequence companions ruled out by SED limit  ($M_*\lesssim1.4~M_\odot$).\\
		 \vspace{1mm}
		 Single WD & \xmark & WD will exceed Chandrasekhar limit ($M_{\rm WD}>1.4~M_\odot$).\\
		 \vspace{1mm}		 
		 Single NS & \xmark & NS will exceed maximum mass ($M_{\rm NS}>2.3~M_\odot$).\\		 
		 \vspace{1mm}		 
		 Single BH & \cmark \cmark & Simplest explanation. \\
		\hline
				 \vspace{1mm}
		 $^{\rm \dagger}$Star + Star & \xmark &  Ruled out by SED limit ($M_{\rm binary}\lesssim2.6~M_\odot$).\\
		 		 \vspace{1mm}
		 $^{\rm \dagger}$Star + WD & \xmark & For $M_*\lesssim1.4~M_\odot$, the WD mass exceeds Chandrasekhar limit. \\		
		 		 \vspace{1mm}
		 $^{\rm \dagger}$Star + NS & \xmark & For $M_*<1.4~M_\odot$, the NS mass exceeds $2.2 M_\odot$.\\
		 		 \vspace{1mm}
		 $^{\rm \dagger}$Star + BH & \xmark & For $M_*<1.4~M_\odot$, the BH mass should be $M_{\rm BH}>2.8~M_\odot$. \\	
		\hline
		 		 \vspace{1mm}		
		 $^{\rm \dagger}$WD + WD & \xmark & Both WD components exceed Chandrasekhar limit. \\
		 		 \vspace{1mm}
		 $^{\rm \dagger}$NS + WD & \xmark & NS mass is in the observed range if $M_{\rm WD}>0.8~M_\odot$ \\	
		 		 \vspace{1mm}
		 $^{\rm \dagger}$BH + WD  & \xmark & BH mass is even lower than with no WD. \\			 		 
		 		 \vspace{1mm}		
		 $^{\rm \dagger}$NS + BH & \xmark & The BH must have a NS-like mass. \\
		 		 \vspace{1mm}		 
		 $^{\rm \dagger}$NS + NS & \xmark & Both NS components should have $M_{\rm NS}\gtrsim1.2~M_\odot$, so $q_{\rm inner}\gtrsim0.67$. \\
		 		 \vspace{1mm}
		 $^{\rm \dagger}$BH + BH & \xmark & The BHs have NS masses. \\

		
\hline
\end{tabular}
    \begin{tablenotes}
      \small
      \item $^{\rm \dagger}$ Disfavored because the orbital motion of an inner binary will dominate over the reflex motion of the giant's orbit observed in our spectra.
    \end{tablenotes}

\end{threeparttable}
\label{tab:scenarios}
\end{table*}



\section{Conclusions}
\label{section:summary}

The evolved red giant 2M04123153+6738486 with $T_{\rm eff, giant}\simeq4150$~K, $L_{\rm giant}\simeq230~L_\odot$ is in a $P=81.2$~d binary with a companion of mass $M_{\rm comp} \simeq3.0~ M_\odot$. The ASAS-SN, ATLAS, \textit{TESS} and ZTF light curves show that 2M0412 is an ellipsoidal variable ($\S$\ref{section:phoebe}, Figure \ref{lcs}). The high-resolution Keck/HIRES and LBT/PEPSI spectra indicate that the giant is rapidly rotating ($\S$\ref{section:phoebe}). If it is tidally synchronized, the orbital inclination is $i_{\rm orb}\simeq40-48^\circ$.

We first modeled the light curves with \verb"ELC" using constraints on the spectroscopic surface gravity, period, radial velocities and stellar temperature, assuming a giant + compact object binary. Our \verb"ELC" models indicate that the giant is (almost) filling its Roche lobe. Next, we ran \verb"PHOEBE" models at fixed radii to derive an inclination of $i=41.9^\circ{}^{+0.1^\circ}_{-0.1^\circ} $, a mass ratio of $q\simeq0.20\pm0.01$, a companion mass of $M_{\rm comp}=2.972^{+0.017}_{-0.015}$ and a giant mass of $M_{\rm giant}=0.595^{+0.002}_{-0.006}~ M_\odot$ at the SED radius of $R_{\rm giant}=29~R_\odot$ ($\S$\ref{section:phoebe}). The mass of the giant indicates that its envelope is heavily stripped due to binary interactions. However, this interpretation is complicated by the detection of a secondary component in the spectra (Figure \ref{specsb2}) and the RV cross-correlation function (Figure \ref{rvccf}), which yields a consistent mass ratio of $q\simeq0.201\pm0.010$ (Figure \ref{rvsb2}) which is entirely consistent with our \verb"PHOEBE" model. While absorption lines due to accretion disks have previously been observed \citep{Strader2016}, they are very rare. Given that this second component apparently traces the reflex motion of the binary, we find it unlikely to be associated with another inner binary.

We also considered a mass transferring giant + star binary ($\S$\ref{section:ccf}). Our \verb"PHOEBE" models give $M_{\rm giant}=0.626^{+0.054}_{-0.049}~M_\odot$, $M_{\rm comp}=2.72^{+0.18}_{-0.18}~M_\odot$, $R_{\rm giant}=30.8^{+0.9}_{-0.9}~R_\odot$, $R_{\rm comp}=8.8^{+1.2}_{-0.9}~R_\odot$, $T_{\rm{eff, giant}}=4240^{+110}_{-140}$~K, $T_{\rm{eff, comp}}=5950^{+170}_{-290}$~K, $i=44.4^{+1.4}_{-1.1}^\circ$, and $q=M_{\rm giant}/M_{\rm comp}=0.232^{+0.007}_{-0.007}$. This interpretation is complicated by the expected luminosity of the companion $L_{\rm comp}\simeq87~L_\odot$, which would be evident in the SED ($\S$\ref{section:giant}, Figure \ref{sedfit}). We also compare the observed properties of this binary to the BPASS binary evolution models and find both giant + compact object and giant + star binaries that match our observations. The BPASS model that best matches our results is a giant + compact object binary where the giant has gone through significant mass loss through Roche Lobe overflow. MESA models of mass transferring giant + star binaries indicate that the accreting companion has to be significantly hotter ($\log T_{\rm eff}\gtrsim4.0$) and more luminous ($\log (L/L_\odot)\gtrsim1.5$) than what is allowed by the SED. However, the companion could also be an unusual mass transfer binary consisting of a giant and a massive star that fall outside the investigated BPASS/MESA models. We find no evidence for a hotter, luminous stellar companion in the SED and can rule out both single and binary main sequence companions to limits of $M_{\rm single}<1.4~M_\odot$ and $M_{\rm binary}<2.6~M_\odot$ ($\S$\ref{section:giant}, Figure \ref{sedfit}).

We also find a broad, phase variable $\rm H\alpha$ emission line ($\S$\ref{section:balmer}, Figure \ref{spechalpha}) which is likely due to an accretion disk. The properties of the $\rm H\alpha$ emission are consistent with Roche lobe overflow from the giant. We derive a \textit{Swift} XRT X-ray flux limit corresponding to $L_{\rm X}\lesssim3.4\times10^{31}~\rm ergs~s^{-1}$ ($L/L_{\rm edd}{\lesssim}10^{-7}$) ($\S$\ref{section:xrays}). The simplest explanation for the companion is a single compact object, most likely a black hole, but possibly a high mass neutron star, in the ``mass gap'' (Table \ref{tab:scenarios}, Figure \ref{masses}). 

\section*{Acknowledgements}

We thank Dr. J. Strader for a careful reading of this manuscript. We thank Dr. J. J. Eldridge for useful discussions on the BPASS models. We thank Las Cumbres Observatory and its staff for their continued support of ASAS-SN. ASAS-SN is funded in part by the Gordon and Betty Moore Foundation through grants GBMF5490 and GBMF10501 to the Ohio State University, and also funded in part by the Alfred P. Sloan Foundation grant G-2021-14192.

TJ, KZS and CSK are supported by NSF grants AST-1814440 and 
AST-1908570. TJ acknowledges support from the Ohio State Presidential Fellowship. TAT is supported in part by NASA grant 80NSSC20K0531. TAT acknowledges previous support from Scialog Scholar grant 24216 from the Research Corporation, from which this effort germinated.  J.T.H. is supported by NASA award 80NSSC21K0136.
D.H. acknowledges support from the Alfred P. Sloan Foundation, the National Aeronautics and Space Administration (80NSSC18K1585, 80NSSC19K0379), and the National Science Foundation (AST-1717000).CB acknowledges support from the National Science Foundation grant AST-1909022.

Parts of this research were supported by the Australian Research Council Centre of Excellence for All Sky Astrophysics in 3 Dimensions (ASTRO 3D), through project number CE170100013 and the Australian Research Council Centre of Excellence for Gravitational Wave Discovery (OzGrav), through project number CE170100004.

Funding for the Sloan Digital Sky Survey IV has been provided by the Alfred P. Sloan Foundation, the U.S. Department of Energy Office of Science, and the Participating Institutions. SDSS-IV acknowledges
support and resources from the Center for High-Performance Computing at
the University of Utah. The SDSS web site is www.sdss.org.

SDSS-IV is managed by the Astrophysical Research Consortium for the 
Participating Institutions of the SDSS Collaboration including the 
Brazilian Participation Group, the Carnegie Institution for Science, 
Carnegie Mellon University, the Chilean Participation Group, the French Participation Group, Harvard-Smithsonian Center for Astrophysics, 
Instituto de Astrof\'isica de Canarias, The Johns Hopkins University, Kavli Institute for the Physics and Mathematics of the Universe (IPMU) / 
University of Tokyo, the Korean Participation Group, Lawrence Berkeley National Laboratory, 
Leibniz Institut f\"ur Astrophysik Potsdam (AIP),  
Max-Planck-Institut f\"ur Astronomie (MPIA Heidelberg), 
Max-Planck-Institut f\"ur Astrophysik (MPA Garching), 
Max-Planck-Institut f\"ur Extraterrestrische Physik (MPE), 
National Astronomical Observatories of China, New Mexico State University, 
New York University, University of Notre Dame, 
Observat\'ario Nacional / MCTI, The Ohio State University, 
Pennsylvania State University, Shanghai Astronomical Observatory, 
United Kingdom Participation Group,
Universidad Nacional Aut\'onoma de M\'exico, University of Arizona, 
University of Colorado Boulder, University of Oxford, University of Portsmouth, 
University of Utah, University of Virginia, University of Washington, University of Wisconsin, 
Vanderbilt University, and Yale University.


This work has made use of data from the European Space Agency (ESA)
mission {\it Gaia} (\url{https://www.cosmos.esa.int/gaia}), processed by
the {\it Gaia} Data Processing and Analysis Consortium. This publication makes 
use of data products from the Two Micron All Sky Survey, as well as
data products from the Wide-field Infrared Survey Explorer.
This research was also made possible through the use of the AAVSO Photometric 
All-Sky Survey (APASS), funded by the Robert Martin Ayers Sciences Fund. 

The LBT is an international collaboration among institutions in the
United States, Italy and Germany. LBT Corporation partners are: The
University of Arizona on behalf of the Arizona Board of Regents;
Istituto Nazionale di Astrofisica, Italy; LBT Beteiligungsgesellschaft,
Germany, representing the Max-Planck Society, The Leibniz Institute for
Astrophysics Potsdam, and Heidelberg University; The Ohio State
University, representing OSU, University of Notre Dame, University of
Minnesota and University of Virginia.

PEPSI was made possible by funding through the State of
Brandenburg (MWFK) and the German Federal Ministry of Education and
Research (BMBF) through their Verbundforschung grants 05AL2BA1/3 and
05A08BAC.

This research is based on observations made with the \textit{Neil Gehrels Swift Observatory}, obtained from the MAST data archive at the Space Telescope Science Institute, which is operated by the Association of Universities for Research in Astronomy, Inc., under NASA contract NAS 5-26555. This paper includes data collected with the \textit{TESS} mission, obtained from the MAST data archive at the Space Telescope Science Institute (STScI). Funding for the TESS mission is provided by the NASA Explorer Program. STScI is operated by the Association of Universities for Research in Astronomy, Inc., under NASA contract NAS 5-26555.

Some of the data presented herein were obtained at the W. M. Keck Observatory, which is operated as a scientific partnership among the California Institute of Technology, the University of California and the National Aeronautics and Space Administration. The Observatory was made possible by the generous financial support of the W. M. Keck Foundation.

Based on observations obtained with the Samuel Oschin Telescope 48-inch and the 60-inch Telescope at the Palomar Observatory as part of the Zwicky Transient Facility project. ZTF is supported by the National Science Foundation under Grant No. AST-2034437 and a collaboration including Caltech, IPAC, the Weizmann Institute for Science, the Oskar Klein Center at Stockholm University, the University of Maryland, Deutsches Elektronen-Synchrotron and Humboldt University, the TANGO Consortium of Taiwan, the University of Wisconsin at Milwaukee, Trinity College Dublin, Lawrence Livermore National Laboratories, and IN2P3, France. Operations are conducted by COO, IPAC, and UW.

The authors wish to recognize and acknowledge the very significant cultural role and reverence that the summit of Maunakea has always had within the indigenous Hawaiian community.  We are most fortunate to have the opportunity to conduct observations from this mountain.

We thank the ZTF and ATLAS projects for making their light curve data publicly available.
This research has made use of the VizieR catalogue access tool, CDS, Strasbourg, France. 
This research also made use of Astropy, a community-developed core Python package for 
Astronomy \citep{astropy:2013,astropy:2018}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Data Availability}

The photometric data are all publicly available. The spectra will be shared on reasonable request to the corresponding author.




%%%%%%%%%%%%%%%%%%%% REFERENCES %%%%%%%%%%%%%%%%%%

% The best way to enter references is to use BibTeX:

\bibliographystyle{mnras}
\bibliography{refbh} % if your bibtex file is called example.bib


% Alternatively you could enter them by hand, like this:
% This method is tedious and prone to error if you have lots of references
%\begin{thebibliography}{99}
%\bibitem[\protect\citeauthoryear{Author}{2012}]{Author2012}
%Author A.~N., 2013, Journal of Improbable Astronomy, 1, 1
%\bibitem[\protect\citeauthoryear{Others}{2013}]{Others2013}
%Others S., 2012, Journal of Interesting Stuff, 17, 198
%\end{thebibliography}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%% APPENDICES %%%%%%%%%%%%%%%u%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Don't change these lines
\bsp	% typesetting comment
\label{lastpage}
\end{document}

% End of mnras_template.tex


==> removedstuff.tex <==

\begin{figure*}
    
    \includegraphics[width=1\textwidth]{bpass_bestgiantcompact.pdf}
    \includegraphics[width=1\textwidth]{bpass_bestgiantstar.pdf}    
    \caption{\textit{Left:} Evolutionary tracks corresponding to the best giant + compact object (top) and giant + star (bottom) BPASS models in the Hertzsprung-Russell diagram. The blue and orange shaded regions show the luminosity and temperature constraints from the SED fit. \textit{Middle:} Evolution of the masses of the two components in the binary and the He core mass. \textit{Right:} Evolution of the stellar radii and the orbital separation. Periods of Roche lobe overflow are shaded in orange. The dot dashed lines indicate the epoch at which the models match the observations.}
    \label{bpassconfig}
\end{figure*}

The stellar evolution tracks, and the evolution of the mass, radii and orbital separation for this model are shown in Figure \ref{bpassconfig}. 

The parameters for the binary orbit, red giant and the companion that we adopt hereafter are summarized in Table \ref{tab:params}.


\begin{table}
\begin{center}
\caption{Adopted parameter estimates for the companion and red giant from PHOEBE modeling. }\label{tab:params}
	\begin{tabular}{r c c c }
	\hline	
	& Parameter & Companion   &   Red giant \\
	\hline
	\vspace{2mm}
	& $P_{\rm orb}$  (d) & \multicolumn{2}{c}{$81.16839^{+0.00044}_{-0.00045}$} \\
	\vspace{2mm}
	& $\omega~(^\circ)$ & \multicolumn{2}{c}{$0$ (fixed)}\\% & $-$ & $-$\\
	\vspace{2mm}
	& $e$ & \multicolumn{2}{c}{$0$ (fixed)}\\%& $-$ & $-$\\
	\vspace{2mm}	
	& $i~(^\circ)$  & \multicolumn{2}{c}{$37.87^{+0.32}_{-0.36}$}\\% &  $-$ & $-$ \\
	\vspace{2mm}
	& $q$ & \multicolumn{2}{c}{$0.261^{+0.019}_{-0.021}$} \\% $-$ & $-$\\	
	\vspace{2mm}
	& ${v_\gamma}~(\rm km ~s^{-1})$ &  \multicolumn{2}{c}{$-47.316^{+0.011}_{-0.010}$}\\% & $-$ & $-$ \\
	\vspace{2mm}
	& $a ~(R_{\odot})$ & $28.6^{+1.9}_{-2.1}$ & $109.3^{+0.9}_{-0.8}$ \\
	\vspace{2mm}	
	& $T_{\rm{eff}}~(K)$ & $300$ (fixed) & $4050^{+100}_{-110}$\\
	\vspace{2mm}
	& $R~(R_{\odot})$ & $3\times 10^{-6}$ (fixed) & $37.2\pm1.1$\\	
	\vspace{2mm}	
	& $M~(M_{\odot})$ & $4.234^{+0.068}_{-0.075}$ & $1.108^{+0.090}_{-0.101}$\\
	\hline
	\vspace{2mm}	
\end{tabular}
\end{center}
\end{table}


The corner plot of the derived component masses and semi-major axis of the binary is shown in Figure \ref{cornerderive}. 

\begin{figure}
	\includegraphics[width=0.5\textwidth]{corner_phoebe_ztf_sd_derived.pdf}
    \caption{The corner plot for the posterior samples for $q$, $i$, $R_{\rm giant}$ and $T_{\rm eff, giant}$ in the best-fitting giant + compact object PHOEBE model to the ZTF $r-$band and \textit{TESS} light curves.}
    \label{cornerderive}
\end{figure}

The best-fit orbit from $\S$\ref{section:phoebe} is shown in Figure \ref{rvs}. 

\begin{figure*}
	\includegraphics[width=0.98\textwidth]{rvs.pdf}
    \caption{The observed radial velocities for 2M0412 as a function of orbital phase, defined with the epoch of maximal RV at $\phi=0.75$ (top). The RVs from APOGEE DR16, Keck/HIRES and LBT/PEPSI are shown as blue circles, red squares and purple diamonds respectively. The best-fit RV fit from the PHOEBE binary models is shown in black and the residuals are shown in the bottom panel. }
    \label{rvs}
\end{figure*}

In summary, by searching the BPASS models, we find binaries consisting of a giant and either another star or a compact object that match the observations and derived properties of 2M0412. We find more giant + compact object binaries than giant + star binaries using our search criteria. The BPASS model that best matches the current properties of the binary is a giant + compact object binary. In both sets of binaries, the giant is going through or has just completed an episode of RLOF. 


\subsection{Interpreting 2M0412 as a giant + star binary}

To interpret 2M0412 as a stellar binary requires that it was a mass transfer system where the observed star is much less massive than estimates for single star evolution. Given that the giant is on the upper RGB and not on the red clump (Figure \ref{loggteff}), the giant will have a degenerate core and so we can place a very firm lower limit to its mass. The luminosity of a giant with a degenerate core of mass $M_{\rm core}$ is
\begin{equation}
    \label{eq:coremass}
    \bigg(\frac{L}{L_\odot}\bigg)\approx 675 \bigg(\frac{M_{\rm core}}{0.4~M_\odot}\bigg)^{7}.
\end{equation} \citep{Boothroyd1988}, so we must have $M_{\rm giant}>M_{\rm core}\simeq0.35~M_\odot$ for $L\sim250~L_\odot$. With the constraint on $q$, this implies a lower bound for the companion mass of $M_{\rm comp}\gtrsim1.75~M_\odot$, larger than the limit for a single stellar companion in $\S$\ref{section:giant} ($M_*\lesssim1.4~M_\odot$, Figure \ref{sedfit}). This suggests that the mass of the companion has to be dominated by a dark, compact component.

We consider the scenario of a stripped low mass giant in a binary with a low mass main sequence star. Using just the dynamical information ($K_{\rm giant}$, $K_{\rm comp}$ and $P_{\rm orb}$), we get $a_{\rm orb}\sin i=(a_{\rm giant}+a_{\rm comp})\sin i=80.4\pm0.2~R_\odot$. Using Kepler's third law, this corresponds to $M_{\rm tot}\sin^3 i=(M_{\rm giant}+M_{\rm comp})\sin^3 i=1.06\pm0.01~M_\odot$. Using the constraint on $q$, we can derive the minimum mass of the giant and the companion as
\begin{equation}
    M_{\rm comp}\sin^3 i=0.88\pm0.01~M_\odot,
\end{equation}
and
\begin{equation}
    M_{\rm giant}\sin^3 i=0.18\pm0.01~M_\odot.
\end{equation} For the giant to have the minimum mass given its luminosity, $M_{\rm giant}=M_{\rm core}\simeq0.35~M_\odot$ (Equation \ref{eq:coremass}), $\sin i =0.80\pm0.01$ and $i=53.1\pm1.0^\circ$. At this inclination, $M_{\rm comp}=1.72\pm0.07~M_\odot$, which is again larger than the single star limit from the SED ($M\gtrsim1.4~M_\odot$). If we assume that the giant has $M_{\rm giant}\simeq1.00~M_\odot$, $\sin i =0.56\pm0.01$ and $i=34.0\pm0.7^\circ$. This implies that $M_{\rm comp}=5.01\pm0.27~M_\odot$. If we were to explain the second component as emerging from a single star with a mass at the SED limit ($M{\sim}1.4~M_\odot$), then $\sin i{\sim}0.86$, $i{\sim}59.3^\circ$ and $M_{\rm giant}{\sim}0.28~M_\odot$, the mass of the giant will be below the mass of the degenerate core ($M_{\rm core}\simeq0.35~M_\odot$). In our best-fitting giant + star \verb"PHOEBE" models, the giant star has a mass of $M_{\rm giant}=0.626^{+0.054}_{-0.049}~ M_\odot$ and its companion has a mass of $M_{\rm comp} =2.720^{+0.180}_{-0.180}~ M_\odot$. The companion is fairly large with $R_{\rm comp}=8.8^{+1.2}_{-0.9}~R_\odot$ and has an effective temperature $T_{\rm{eff, comp}}=5950^{+170}_{-290}$~K. 

We use Modules for Experiments in Stellar Astrophysics \citep[MESA][]{Paxton2011, Paxton2013, Paxton2015, Paxton2018, Paxton2019} to investigate the evolution of a binary that could result in a 2M0412-like system with a giant and a stellar companion. The MESA EOS is a blend of the OPAL \citet{Rogers2002}, SCVH \citet{Saumon1995}, PTEH \citet{Pols1995}, HELM \citet{Timmes2000}, and PC \citet{Potekhin2010} EOSes. Radiative opacities are primarily from OPAL \citep{Iglesias1993, Iglesias1996}, with low-temperature data from \citet{Ferguson2005} and the high-temperature, Compton-scattering dominated regime by \citet{Buchler1976}. Electron conduction opacities are from \citet{Cassisi2007}. Nuclear reaction rates are a combination of rates from NACRE \citep{Angulo1999}, JINA REACLIB \citep{Cyburt2010}, plus additional tabulated weak reaction rates \citet{Fuller1985, Oda1994, Langanke2000}. Screening is included via the prescription of \citet{Chugunov2007}. Thermal neutrino loss rates are from \citet{Itoh1996}. MESA computes Roche lobe radii in binary systems using the fit of \citet{Eggleton1983}, and the mass transfer rates in Roche lobe overflowing binary systems are determined following the prescription of \citet{Kolb1990}. We adopt the explicit mass transfer calculation scheme in MESA.

We evolve the BPASS giant + star binaries (Models 1-3, Table \ref{tab:bpass}) with MESA to investigate the properties of the accretor when the binary is at an orbital period similar to 2M0412 (${\sim}81$~days). We use the initial component masses and orbital period ($P_{\rm orb,init}=25.2$~days) from the BPASS models. When the binary is at $P_{\rm orb}{\sim}81$~days, the initially more massive component is a red giant with $M_{\rm giant}\simeq0.57-0.65~M_\odot$ and its companion is a main sequence star with $M_{\rm comp}\simeq2.09-2.39~M_\odot$, matching the BPASS results. The giant has $T_{\rm eff, giant}\simeq4094-4103$~K, $R_{\rm giant}\simeq28.7-30.2~R_\odot$, $\log(g)\simeq1.3$ and $L_{\rm giant}\simeq209-232~L_\odot$. The giant is in the process of transferring mass to its companion, with the whole mass transfer episode lasting ${\sim}49-58$~Myr. Once the mass transfer is complete, the binary is at an orbital period of $P_{\rm orb}\simeq220-281$~days and the giant is stripped significantly and the accretor having gained a significant amount of mass. 

The companion to the giant is hot, compact and luminous, with $T_{\rm eff, comp}\simeq10800-11700$~K, $R_{\rm comp}\simeq1.6-1.8~R_\odot$, $\log(g)\simeq4.3$ and $L_{\rm comp}\simeq35-57~L_\odot$. Such a hot companion is grossly incompatible with the NUV limits from \textit{Swift} and \textit{GALEX} ($\S$\ref{section:giant}, Figure \ref{sedbpass}). This is also significantly hotter than the temperature derived for the second component from fitting the spectra ($T_{\rm{eff, comp}}=6347\pm700$~K), \verb"PHOEBE" models ($T_{\rm{eff, comp}}=5950^{+170}_{-290}$~K) and the BPASS models ($T_{\rm{eff, comp}}=6270-6870$~K). The luminosity derived for the second component in the best fitting giant + star \verb"PHOEBE" model ($L_{\rm comp}\simeq87~L_\odot$) is somewhat larger than the luminosity of the companion in the MESA models, and the radius of the companion from MESA is significantly smaller than the estimate from \verb"PHOEBE".

\begin{table*}
	\centering
	\caption{Properties of the MESA binary models for the giant + star binaries in BPASS that match observations for 2M0412. The initial masses of the stars are listed as $M_1$ and $M_2$. The MESA binaries are evolved from an initial orbital period of 25.2~days.}

\begin{threeparttable}	
\begin{tabular}{rrrrrrrrrrrrrr}
		\hline
		\vspace{1mm}	
		 Model & $M_{1}$  & $M_{2}$ & $M_{\rm giant}$  & $M_{\rm comp}$ & $q$ & $T_{\rm eff, giant}$ & $T_{\rm eff, comp}$ & $R_{\rm giant}$ & $R_{\rm comp}$  & $L_{\rm giant}$ & $L_{\rm comp}$ & $P_{\rm orb}$ & Age\\
		 
		  & $(M_{\odot})$ & $(M_{\odot})$ & $(M_{\odot})$ & $(M_{\odot})$ & & (K) & (K) & $(R_{\odot})$ & $(R_{\odot})$ & $(L_{\odot})$ & $(L_{\odot})$ &  $(\rm d)$ &  Gyr\\		 
		\hline
        1 & 1.60 & 1.28 &0.61 & 2.27 & 0.270 & 4096 & 11692 & 29.4 & 1.6 & 220 & 43  & 81.10 & 1.7\\
        2 & 1.40 & 1.26 & 0.57& 2.09 & 0.274 & 4094 & 10780 & 28.7 & 1.7 & 209 & 35 & 81.16 & 2.6\\         
        3 & 1.60 & 1.44 & 0.65 & 2.39 & 0.274 & 4103 & 11730 & 30.2 & 1.8 & 232 & 57  & 81.12 & 1.7\\
		\hline
\end{tabular}


\end{threeparttable}
\label{tab:mesa}
\end{table*}


Interpreting 2M0412 as a giant + star binary is problematic. The \verb"PHOEBE" models indicate a large luminosity for the companion $L_{\rm comp}\simeq87~L_\odot$, which is clearly not present given the SED (Figure \ref{sedfit}. Additionally, our MESA models of mass transferring giant + star binaries indicate that the accreting star should be significantly hotter ($T_{\rm eff, comp}\simeq10800-11700$~K) and more compact ($R_{\rm comp}\simeq1.6-1.8~R_\odot$) than the estimates from \verb"PHOEBE" and the spectrum of the second component ($\S$\ref{section:ccf}). For the companion to be consistent with the SED, the luminosity should be $\lesssim25~L_\odot$ (a factor of ${\sim}3.5\times$ smaller than the \verb"PHOEBE" estimate and a factor of ${\sim}1.4-2.3\times$ smaller than the estimates from MESA). A main sequence star (as predicted by the MESA models) is ruled out by the SED limits, with $M_{\rm comp} < 1.4~ M_\odot$, and such a star cannot account for the total mass of the companion while having a temperature below the SED limit. 

%To investigate the properties of the accretor, we use the initial conditions from the BPASS giant + star models to evolve binaries using MESA. We find that the accreting star has to be significantly hotter ($T_{\rm eff, comp}\simeq10800-11700$~K) than what is observed as the second component in our spectra ($T_{\rm{eff, comp}}=6347\pm700$~K).

\subsection{Interpreting 2M0412 as a giant + compact object binary}

The other option is that the companion is a compact object. Using the luminosity of the giant, we were able to place a very firm lower limit on the mass of the giant of $M_{\rm giant}>M_{\rm core}\simeq0.35~M_\odot$ (Equation \ref{eq:coremass}). Given the binary mass function $f(M)\simeq0.58~M_\odot$ (Table \ref{tab:orbit}) and assuming an edge-on orbit, we can place a firm lower bound on the companion's mass of $M_{\rm comp}\gtrsim1.04~M_\odot$. We can exclude orbital inclinations larger than $i_{\rm orb}{\simeq}50^\circ$ based on the differences in the depths between the primary and secondary minima in the observed light curves \citep{Morris1993}. If $i_{\rm orb}\lesssim50^\circ$, the companion must have $M_{\rm comp}\gtrsim1.83~M_\odot$. A MS companion of this mass is easily ruled out with the SED and UV upper limits ($\S$\ref{section:giant}). Based on the SED we estimate $M_{\rm giant}=1.11^{+0.24}_{-0.22}~M_\odot$, leading to $M_{\rm comp}\gtrsim2.6~M_\odot$ for $i_{\rm orb}\lesssim50^\circ$. For the \verb"PHOEBE" models of a giant + compact object binary without veiling, we find $M_{\rm giant}=1.108^{+0.090}_{-0.101}~ M_\odot$ and $M_{\rm comp} =4.234^{+0.068}_{-0.075}~ M_\odot$. 

Our \verb"ELC" and \verb"PHOEBE" models indicate that the giant is filling (or almost filling) its Roche lobe. Additionally, the presence of $\rm H\alpha$ emission strongly supports this semi-detached orbital configuration, therefore, we can independently derive the mass of the giant from the period--density relationship for semi-detached binaries. Roche lobe filling stars at a given orbital period will have nearly the same mean density \citep{Eggleton1983,El-Badry2021}, which can be expressed as
\begin{equation}
    \bar{\rho}\approx0.185~ {\rm g~cm^{-3}} \bigg(\frac{P_{\rm orb}}{\rm days}\bigg)^{-2}=2.8\times10^{-5}~{\rm g~cm^{-3}}\bigg(\frac{P_{\rm orb}}{\rm 81~ days}\bigg)^{-2}.
\end{equation} This density clearly implies that the star is a giant. We can derive the mass of the giant for a given stellar radius as,
\begin{equation}
    M_{\rm giant}=4\pi/3~R_{\rm giant}^3~\bar{\rho}\approx0.6~ M_\odot \bigg(\frac{R_{\rm giant}}{\rm 31~ R_\odot}\bigg)^{3} \bigg(\frac{P_{\rm orb}}{\rm 81~ days}\bigg)^{-2}.
\end{equation} Using the binary mass function and assuming an edge on orbit, $M_{\rm comp}\simeq1.3~M_\odot$. Using the constraint on $q$ from the radial velocities ($\S$\ref{section:ccf}), $M_{\rm comp}\simeq3.0~M_\odot$, which implies $i=41^\circ$, consistent with the inclination estimated from $v_{\rm rot} \, \textrm{sin} \, i$ measurements. The \verb"ELC" and \verb"PHOEBE" models for a giant + compact object binary yield larger radii, with $R_{\rm giant}=35-37~R_\odot$, which implies $M_{\rm giant}\simeq0.9-1.0~M_\odot$ and $M_{\rm comp}\simeq4.5-5.0~M_\odot$. Even if we assume the smaller radius estimate from the SED ($\S$\ref{section:giant}), the companion is fairly massive with $M_{\rm comp}\simeq3.0~M_\odot$ and a simple main sequence star of this mass is easily ruled out by the SED. 

%Using the dynamical information, including the dynamics of the second component in the spectra ($\S$\ref{section:ccf}), we have also explored a binary scenario with a stripped red giant and a main sequence star, but we find that if the component is a main sequence star that has a mass smaller than the SED limit of $M_{\rm comp} < 1.4 M_\odot$, the mass of the giant is smaller than the mass of the degenerate core $M_{\rm core}\simeq0.35~M_\odot$. At the limit where $M_{\rm giant}=M_{\rm core}\simeq0.35~M_\odot$, the mass of the companion is larger than the single star SED limit. The BPASS models ($\S$\ref{section:bpass}) that match this system all have stripped giants, but all of them have $M_{\rm giant}>0.48~M_\odot$. For 2M0412, we adopt $M_{\rm giant}\simeq0.6~M_\odot$ as a lower limit based on the radius derived from the SED and the giant filling its Roche Lobe. The binary modeling yield giant masses larger than this limit. 
%A red giant with a mass $M_{\rm giant}\simeq0.9-1~M_\odot$ is a better choice and is consistent with observational constraints from the spectra, SED and our binary models in $\S$\ref{section:phoebe}. 

Figure \ref{masses} summarizes our discussion on the masses of the companion and the giant. Lower mass giants $M_{\rm giant}\lesssim0.6~M_\odot$ are all essentially ruled out if the giant fill its Roche lobe. We highlight five different estimates of the giant and companion masses in Figure \ref{masses}. The three \verb"PHOEBE" models are summarized in Table \ref{tab:phoebefits} and Table \ref{tab:phoebefitsstripped}. The two \verb"ELC" models are summarized in $\S$\ref{section:phoebe}, $\S$\ref{section:ccf} and Table \ref{tab:elcfits}. One of the \verb"ELC" models highlighted here includes an accretion disk, and when compared to the other models, yields lower mass estimates for the giant and companion of $M_{\rm giant}=0.72^{+0.04}_{-0.03}~M_\odot$, and $M_{\rm comp}=3.11^{+0.11}_{-0.08}~M_\odot$. The smallest mass estimates come from modeling a giant + star binary with \verb"PHOEBE", where $M_{\rm giant}=0.626^{+0.054}_{-0.049}~ M_\odot$ and $M_{\rm comp} =2.720^{+0.180}_{-0.180}~ M_\odot$. All lines of evidence (Roche limits/period--density relation, spectroscopic mass ratio, etc.) and all the binary models indicate that the companion is fairly massive with $M_{\rm comp}\gtrsim2.7~M_\odot$.


If the companion is a single object, the options are a star, a white dwarf (WD), a neutron star (NS) or a black hole (BH). We summarize all the possible scenarios for the composition of the companion if it is a compact object in Table~\ref{tab:scenarios}. A WD is ruled out because its mass would exceed the Chandrasekhar mass limit of $1.4 M_\odot$. A NS is also ruled out since the companion mass exceeds the maximum possible mass of a neutron star ($M\sim3~M_\odot$; \citealt{Lattimer2001}). Thus, if we only consider 2M0412 to be a giant + star binary, the simplest explanation for the companion to the red giant is a black hole in the low mass gap. However, this interpretation is complicated by the second set of absorption lines in the spectra. While not unprecedented \citep{Strader2016}, absorption lines that emerge from accretion disks around compact objects are very rare.


\begin{figure*}
    
    \includegraphics[width=\textwidth]{massplot.png}
    \caption{The mass of the companion ($M_{\rm comp}$) as a function of the mass of the giant ($M_{\rm giant}$). The binary mass function at inclinations of $i=90^\circ$, $40^\circ$ and $30^\circ$ are shown as the blue dashed lines. Giants with radii of $R=31~R_\odot$ or $R=35~R_\odot$ will overfill their Roche loves if they have masses less than the Roche limits given by the dashed curve. The companion masses for a mass ratio of $q=0.2$ and $q=0.3$ are shown as the red lines. The black dotted line at $M_{\rm comp}=3~M_\odot$ is shown as a reference. The orange shaded region highlights giant masses that are not allowed by the condition $M_{\rm giant}\gtrsim M_{\rm core}\simeq0.35~M_\odot$. The green shaded region shows companion masses for luminous stars that are allowed by the single star SED limit ($M_*\lesssim1.4~M_\odot$). The derived values for $M_{\rm comp}$ and $M_{\rm giant}$ from various PHOEBE and ELC models are shown in black.}
    \label{masses}
\end{figure*}

Next we investigate the possible scenarios if the companion is a binary. These triple solutions likely require a complex evolutionary pathway which we will not attempt to explore here. All triple solutions are disfavored by the dominance of the reflex motion of the giant's orbit in the second RV component. The companion cannot be a stellar binary given that the two star mass limit from the SED models is $M_{\rm binary}<2.6~M_\odot$. Combining a star with a compact object also seems unlikely because the star will have a high orbital velocity since $M_*<<M_{\rm comp}$ (see $\S$\ref{section:ccf}). For example, an equal mass stellar binary with two $1.3~M_\odot$ stars will have an orbital motion of ${\sim}41\, \rm km \,s^{-1}$ for $i=40^\circ$, much larger than the observed reflex motion of ${\sim}8.3\, \rm km \,s^{-1}$. A double WD binary can be ruled out because each WD will have a mass that exceeds the Chandrasekhar limit.  Combining a WD and a NS seems unlikely because the NS mass must be $>2.8~ M_\odot$ for the WD to have a mass below the Chandrasekhar limit. A double NS binary is unlikely because both NSs will have masses close to to the maximum observed NS masses. BH plus NS or WD binaries are possible but drive the BH mass further into the mass gap. A double BH binary seem implausible because they both require BH masses in the range observed for neutron stars. The simplest explanation is again that the dark companion is a mass gap black hole.

%With the single star SED limit of $<1.4~ M_\odot$, the compact object mass must be $>2.8~ M_\odot$. 



\begin{table*}
	\centering
	\caption{Comparison of the possible scenarios involving stellar companions (*), white dwarfs (WD), neutron stars (NS) and black holes (BH) that can explain the nature of the companion. We assumed $M_{\rm comp}=4.2\pm 0.1~M_\odot$ from $\S$\ref{section:phoebe}. A `\cmark' indicates that the scenario is possible, a `?' indicates that while the scenario is technically possible, it is very unlikely and a `\xmark' indicates that the scenario is ruled out. The simplest explanation is that of a single low mass black hole, indicated with `\cmark \cmark'.}
\begin{threeparttable}	
\begin{tabular}{rrr}
		\hline
		 Dark Companion & Possibility & Comment \\
		 \hline
		 \vspace{1mm}		 
		 Single Star & \xmark & Ruled out by SED limit  ($M_*\lesssim1.4~M_\odot$). \\
		 \vspace{1mm}
		 Single WD & \xmark & WD will exceed Chandrasekhar limit ($M_{\rm WD}>1.4~M_\odot$).\\
		 \vspace{1mm}		 
		 Single NS & \xmark & NS will exceed maximum mass ($M_{\rm NS}>3~M_\odot$).\\		 
		 \vspace{1mm}		 
		 Single BH & \cmark \cmark & Simplest explanation. \\
		\hline
				 \vspace{1mm}
		 $^{\rm \dagger}$Star + Star & \xmark &  Ruled out by SED limit ($M_{\rm binary}\lesssim2.6~M_\odot$).\\
		 		 \vspace{1mm}
		 $^{\rm \dagger}$Star + WD & \xmark & For $M_*\lesssim1.4~M_\odot$, the WD mass exceeds Chandrasekhar limit. \\		
		 		 \vspace{1mm}
		 $^{\rm \dagger}$Star + NS & \xmark & For $M_*<1.4~M_\odot$, the NS mass exceeds $2.2 M_\odot$.\\
		 		 \vspace{1mm}
		 $^{\rm \dagger}$Star + BH & \xmark & For $M_*<1.4~M_\odot$, the BH mass should be $M_{\rm BH}>2.8~M_\odot$. \\	
		\hline
		 		 \vspace{1mm}		
		 WD + WD & \xmark & Both WD components exceed Chandrasekhar limit. \\
		 		 \vspace{1mm}
		 NS + WD & \xmark & NS mass has to be $M_{\rm NS}>2.8~M_\odot$ for the WD mass to be below the Chandrasekhar limit. \\	
		 		 \vspace{1mm}
		 BH + WD  & \cmark & BH mass will be $M_{\rm BH}>2.8~M_\odot$ for $M_{\rm WD}<1.4~M_\odot$.  \\		 		 
		 		 \vspace{1mm}		
		 NS + BH & ? & $2.1~M_\odot<M_{\rm BH}<2.8~M_\odot$ for $1.4~M_\odot<M_{\rm BH}<2.1~M_\odot$. \\
		 		 \vspace{1mm}		 
		 NS + NS & ? & Both NS components should have $M_{\rm NS}\sim2.1~M_\odot$. \\
		 		 \vspace{1mm}
		 BH + BH & \xmark & The BHs have NS masses. \\

		
\hline
\end{tabular}
    \begin{tablenotes}
      \small
      \item $^{\rm \dagger}$ Disfavored because the orbital motion of an inner binary will dominate over the reflex motion of the giant's orbit observed in our spectra.
    \end{tablenotes}

\end{threeparttable}
\label{tab:scenarios}
\end{table*}



\begin{figure}
	\vspace{-2cm}
	\includegraphics[width=0.5\textwidth]{sed_bpass.pdf}
	\vspace{-2cm}
    \caption{The SED model for 2M0412 (black) compared to the SEDs for the companion stars of the giant + star BPASS binaries in Table \ref{tab:bpass} (red). The combined SEDs for the giant and companion star are shown as red dashed lines. The $1\sigma$ \textit{Swift} \textit{UVM2} and \textit{GALEX} \textit{FUV/NUV} upper limits are shown as arrows. \textbf{REPLACE WITH SEDs FOR MESA STARS.} }
    \label{sedbpass}
\end{figure}




\begin{table*}
	\centering
	\caption{Summary of the orbital and component parameters from the ELC models for a giant + compact object binary.}
	\label{tab:elcfits}
\begin{tabular}{rrrr}
		\hline
		 Parameter & ZTF $r$+TESS $T$ & ZTF $r$+ZTF $g$+ TESS $T$ & ZTF $r$+TESS $T$ + Second RV\\
		\hline
	
	\vspace{2mm}
	$T_{\rm eff, giant}~(\rm K)$ & $3870^{+13}_{-9}$ &  $3873^{+10}_{-9}$  &  $3868^{+14}_{-9}$\\	
	\vspace{2mm}	
	$i_{\rm orb}~(^\circ)$ & $35.47^{+1.00}_{-0.5}$ & $36.90^{+3.76}_{-0.76}$  & $35.21^{+0.23}_{-0.21}$\\	
	\vspace{2mm}
	$q_{\rm orb}$ & $0.249^{+0.034}_{-0.051}$ & $0.249^{+0.036}_{-0.049}$ & $0.199^{+0.073}_{-0.042}$\\
	\vspace{2mm}
	$K_{\rm giant} ~(\rm km~ s^{-1})$  & $41.987^{+0.020}_{-0.020}$ & $41.965^{+0.026}_{-0.035}$ & $42.050^{+0.020}_{-0.018}$\\	
	\vspace{2mm}
	${v_\gamma}~(\rm km~ s^{-1})$  &  $-47.257^{+0.007}_{-0.008}$ &  $-47.263^{+0.009}_{-0.011}$ &  $-47.286^{+0.006}_{-0.007}$\\	
	\vspace{2mm}
	$R_{\rm giant}$ $(R_{\odot})$  & $35.7^{+0.2}_{-0.4}$ & $35.6^{+0.3}_{-0.5}$& $36.2^{+0.5}_{-0.5}$\\
	\hline
	\vspace{2mm}		
	$P_{\rm orb} (\rm d)$ & $81.2~\rm d$ (fixed) & $81.2~\rm d$ (fixed) & $81.2~\rm d$ (fixed)\\		
	\vspace{2mm}	
	$e_{\rm orb}$ & $0$ (fixed) & $0$ (fixed) & $0$ (fixed)\\
		\hline
	\vspace{2mm}	
	$M_{\rm giant}~(M_{\odot})$  &  $0.988^{+0.022}_{-0.037}$ &  $1.011^{+0.041}_{-0.044}$&  $1.021^{+0.039}_{-0.040}$\\
	\vspace{2mm}	
	$M_{\rm comp}~(M_{\odot})$  &  $4.673^{+0.123}_{-0.228}$ &  $4.346^{+0.175}_{-0.612}$&  $4.801^{+0.060}_{-0.066}$\\
		\hline	
	\vspace{2mm}		
	$L_{\rm system}~(L_{\odot})$  &  $258^{+4}_{-7}$ &  $258^{+5}_{-7}$ &  $264^{+8}_{-8}$\\	
	\vspace{2mm}
	$f=R_{\rm giant}/R_{\rm Roche, giant}$  &  $0.96^{+0.04}_{-0.03}$ &  $0.92^{+0.02}_{-0.06}$  &  $1.00^{+0.00}_{-0.00}$\\		
\hline
\end{tabular}
\end{table*}


\begin{table*}
	\centering
	\caption{Summary of the orbital and component parameters from the PHOEBE models for a giant + compact object binary.}
	\label{tab:phoebefits}
\begin{tabular}{rrrrrr}
		\hline
		 Parameter & ZTF $r$+TESS $T$ & ZTF $r$+TESS $T$ & ZTF $r$+TESS $T$ & ZTF $r$+ZTF $g$+ TESS $T$ & ZTF $r$+TESS $T$ + Second RV \\
		\hline
	\vspace{2mm}		
	$P_{\rm orb} (\rm d)$ & $81.16839^{+0.00044}_{-0.00045}$ & $81.16839^{+0.00040}_{-0.00043}$ & $81.16851^{+0.00045}_{-0.00045}$ & $81.16842^{+0.00045}_{-0.00042}$ & $81.16892^{+0.00041}_{-0.00046}$\\
	\vspace{2mm}	
	$T_{\rm eff, giant}~(\rm K)$ & $4050^{+100}_{-110}$ &  $4060^{+100}_{-100}$ & $4128^{+97}_{-105}$ & $4048^{+95}_{-103}$ & $4150^{+110}_{-110}$\\	
	\vspace{2mm}	
	$i_{\rm orb}~(^\circ)$ & $37.87^{+0.32}_{-0.36}$ & $40.96^{+0.34}_{-0.33}$ & $44.93^{+0.38}_{-0.43}$ & $37.72^{+0.34}_{-0.32}$ & $37.31^{+0.23}_{-0.22}$\\	
	\vspace{2mm}
	$q_{\rm orb}$ & $0.261^{+0.019}_{-0.021}$ & $0.294^{+0.015}_{-0.014}$ & $0.339^{+0.009}_{-0.017}$ & $0.255^{+0.020}_{-0.020}$ & $0.221^{+0.007}_{-0.011}$\\
	\vspace{2mm}
	$a_{\rm giant}\sin i$ $(R_{\odot})$  & $67.103^{+0.029}_{-0.028}$ & $67.097^{+0.029}_{-0.026}$ & $67.104^{+0.025}_{-0.029}$ & $67.095^{+0.029}_{-0.028}$ & $67.062^{+0.027}_{-0.028}$\\	
	\vspace{2mm}
	${v_\gamma}~(\rm km~ s^{-1})$  &  $-47.316^{+0.011}_{-0.010}$ &  $-47.320^{+0.011}_{-0.012}$ & $-47.326^{+0.012}_{-0.012}$ & $-47.314^{+0.010}_{-0.012}$ & $-47.302^{+0.011}_{-0.010}$\\	
	\hline	
	\vspace{2mm}	
	$e_{\rm orb}$ & $0$ (fixed) & $0$ (fixed) & $0$ (fixed) & $0$ (fixed) & $0$ (fixed)\\
	\vspace{2mm}
	Veiling flux & $0\%$ (fixed) & $10\%$ (fixed) & $20\%$ (fixed) & $0\%$ (fixed) & $0\%$ (fixed)\\	
	\vspace{2mm}
	$f=R_{\rm giant}/R_{\rm Roche, giant}$ & $1$ (fixed) & $1$ (fixed) & $1$ (fixed) & 1 (fixed) & 1 (fixed)\\		
	\hline	
	\vspace{2mm}	
	$M_{\rm giant}~(M_{\odot})$  &  $1.108^{+0.090}_{-0.101}$ &  $1.075^{+0.069}_{-0.066}$ & $1.054^{+0.042}_{-0.063}$ & $1.076^{+0.101}_{-0.098}$ & $0.908^{+0.038}_{-0.051}$\\
	$M_{\rm comp}~(M_{\odot})$  &  $4.234^{+0.068}_{-0.075}$ &  $3.655^{+0.071}_{-0.060}$ & $3.115^{+0.056}_{-0.056}$ & $4.226^{+0.075}_{-0.073}$ & $4.106^{+0.058}_{-0.061}$\\
	\hline
	\vspace{2mm}
	$R_{\rm giant}$ $(R_{\odot})$  & $37.2^{+1.1}_{-1.1}$ & $37.0^{+0.6}_{-0.8}$ & $36.8^{+0.6}_{-0.8}$ & $36.8^{+1.1}_{-1.1}$ & $34.8^{+0.4}_{-0.5}$\\
	\vspace{2mm}	
	$a_{\rm orb}$ $(R_{\odot})$  & $137.9^{+1.2}_{-1.4}$ & $132.4^{+1.3}_{-1.0}$ & $127.0^{+1.0}_{-1.2}$ & $137.5^{+1.4}_{-1.3}$ & $135.0^{+0.8}_{-0.9}$\\
	\vspace{2mm}
	$a_{\rm comp}$ $(R_{\odot})$  & $28.6^{+1.9}_{-2.1}$ & $30.1^{+1.4}_{-1.4}$ & $32.1^{+0.8}_{-1.5}$ & $27.9^{+2.0}_{-2.0}$ & $24.5^{+0.8}_{-1.2}$\\
	\vspace{2mm}
	$a_{\rm RG}$ $(R_{\odot})$  & $109.3^{+0.9}_{-0.8}$ & $102.3^{+0.7}_{-0.7}$ & $95.0^{+0.7}_{-0.6}$ & $109.7^{+0.8}_{-0.8}$ & $110.7^{+0.6}_{-0.6}$\\		
\hline
\end{tabular}
\end{table*}
%The corner plot of the posterior samples for $q$, $i$, $v_\gamma$, $a_{\rm giant}\sin i$ and $T_{\rm eff, giant}$ is shown in Figure \ref{cornerfit}. 


``Veiling'' can result in an underestimated orbital inclination and thus an overestimate of the companion mass. The contribution of the veiling component typically falls off at longer wavelengths (e.g., \citealt{Hynes2005,Jianfeng2015,Jayasinghe2021}), which is an additional reason to focus on the ZTF $r$-band and TESS $T$-band light curves. In $\S$\ref{section:giant}, we estimated the veiling fluxes in the $r$ band as ${\sim}7\%$ using the HIRES spectra. The veiling in the \textit{TESS} band was found to be negligible. We ran additional \verb"PHOEBE" models including veiling fluxes of $F_2=10\%$ and $20\%$ for both the ZTF and TESS bands. These results are listed in Table \ref{tab:phoebefits}. When comparing the models with $F_2=0\%$, $10\%$ and $20\%$ veiling flux, the mass of the red giant is consistent at $M_{\rm giant}\simeq1.1~M_\odot$ but the mass of the companion drops from $M_{\rm comp}\simeq4.2~M_\odot$ for $F_2=0\%$ to $M_{\rm comp}\simeq3.1~M_\odot$ for $F_2=20\%$. At $F_2=20\%$, the orbital inclination is underestimated by ${\sim}7^\circ$. The models without veiling had marginally better $\chi^2$ than the ones where we included veiling flux.


\begin{figure*}
	\includegraphics[width=\textwidth]{corner_phoebe_ztf_sd_fitted.pdf}
    \caption{The corner plot for the posterior samples for $q$, $i$, $R_{\rm giant}$ and $T_{\rm eff, giant}$ in the best-fitting giant + compact object PHOEBE model to the ZTF $r-$band and \textit{TESS} light curves.}
    \label{cornerfit}
\end{figure*}


Using both \verb"ELC" and \verb"PHOEBE", we also fit the RVs of the second component along with the RVs of the giant, the ZTF $r$-band light curve, and the \textit{TESS} $T$-band light curve (see Table \ref{tab:elcfits}). We include a Gaussian prior on the mass ratio based on the above constraint. The resulting parameters of $M_{\rm giant}=0.908^{+0.038}_{-0.051}~M_\odot$, $M_{\rm comp}=4.106^{+0.058}_{-0.061}~M_\odot$ are largely consistent with those obtained in $\S$\ref{section:phoebe}. When the RVs of the second component are fit, the resulting mass estimates for the giant and the companion are slightly lower than the best-fit results that do not consider the RVs of the second component.

These results are summarized in Table \ref{tab:phoebefitsstripped}. 

\begin{table}
	\centering
	\caption{Summary of the orbital and component parameters from the PHOEBE models for a giant + star binary. Here we fit both RV curves.}
	\label{tab:phoebefitsstripped}
\begin{tabular}{rrr}
		\hline
		 Parameter & ZTF $r$+TESS $T$ & ZTF $r$+ZTF $g$+ TESS $T$ \\
		\hline
	\vspace{2mm}		
	$P_{\rm orb} (\rm d)$ & $81.16897^{+0.00044}_{-0.00042}$ & $81.16899^{+0.00040}_{-0.00048}$ \\
	\vspace{2mm}	
	$T_{\rm eff, giant}~(\rm K)$ & $4240^{+110}_{-140}$ &  $4210^{+100}_{-100}$\\	
	\vspace{2mm}
	$T_{\rm eff, comp}~(\rm K)$ & $5950^{+170}_{-290}$ &  $5690^{+180}_{-180}$\\	
	\vspace{2mm}	
	$R_{\rm comp}$ $(R_{\odot})$  & $8.8^{+1.2}_{-0.9}$ & $9.7^{+0.7}_{-0.7}$\\		
	\vspace{2mm}	
	$i_{\rm orb}~(^\circ)$ & $44.40^{+1.40}_{-1.10}$ & $44.85^{+1.28}_{-0.84}$\\	
	\vspace{2mm}
	$q_{\rm orb}$ & $0.232^{+0.007}_{-0.007}$ & $0.234^{+0.012}_{-0.008}$\\
	\vspace{2mm}
	$a_{\rm giant}\sin i$ $(R_{\odot})$  & $67.018^{+0.024}_{-0.028}$ & $67.013^{+0.030}_{-0.033}$ \\	
	\vspace{2mm}
	${v_\gamma}~(\rm km~ s^{-1})$  &  $-47.310^{+0.011}_{-0.010}$ &  $-47.313^{+0.011}_{-0.012}$ \\	
	\hline	
	\vspace{2mm}	
	$e_{\rm orb}$ & $0$ (fixed) & $0$ (fixed) \\
	\vspace{2mm}
	$f=R_{\rm giant}/R_{\rm Roche, giant}$ & $1$ (fixed) & $1$ (fixed)\\		
	\hline	
	\vspace{2mm}	
	$M_{\rm giant}~(M_{\odot})$  &  $0.626^{+0.054}_{-0.049}$ &  $0.622^{+0.041}_{-0.043}$ \\
	$M_{\rm comp}~(M_{\odot})$  &  $2.720^{+0.180}_{-0.180}$ &  $2.660^{+0.120}_{-0.170}$ \\
	\hline
	\vspace{2mm}
	$R_{\rm giant}$ $(R_{\odot})$  & $30.8^{+0.9}_{-0.9}$ & $30.8^{+0.7}_{-0.7}$\\
	\vspace{2mm}	
	$a_{\rm orb}$ $(R_{\odot})$  & $118.0^{+2.6}_{-2.8}$ & $117.2^{+1.9}_{-2.6}$ \\
	\vspace{2mm}
	$a_{\rm comp}$ $(R_{\odot})$  & $22.2^{+0.9}_{-0.9}$ & $22.2^{+0.9}_{-0.8}$\\
	\vspace{2mm}
	$a_{\rm RG}$ $(R_{\odot})$  & $95.7^{+2.0}_{-2.3}$ & $95.0^{+1.4}_{-2.1}$\\		
\hline
\end{tabular}
\end{table}

%As a second, independent fit we use the \textsc{Yorbit} genetic algorithm \citep{Segransan2011}. It has been typically used in the discovery of extra-solar planets (e.g. \citealt{Mortier2016,Martin2019}). As a brief summary, 4800 ``genomes'' are created, where each one represents a fit to the data (amplitude, systemic velocity, phase, period, eccentricity and apsidal alignment). These are then left to evolve through crossovers and mutations until an optimal parameter space is found. The advantage of such an algorithm is that it can efficiently span a large parameter space without needing prior constraints. For example, the eccentricity is only constrained by a maximum of 1 and the period is only constrained by a maximum of half the observation timespan. After the optimal region is found \textsc{Yorbit} applies a final Levenberg-Marquardt routine to find the minimal $\chi^2$ and calculate errorbars through bootstrapping. 

%The result of our fit is shown in Fig. BLAH, and the parameters are shown in BLAH.

%\textsc{Yorbit} will always return some eccentricity, even if insignificant as it is in this case: $e=0.0067 \pm 0.0055$, where this is a $1\sigma$ error. Forcing the fit to be circular actually slightly improves the reduced $\chi^2$ from 53.3 to 50.3. So, overall, we are confident that the orbit is circular, at least to the degree that the observational precision and scatter allow. The observed scatter (and hence why the reduced $\chi^2$ is greater than 1) may be because the APOGEE radial velocity errors are underestimated. Alternatively, there may be some astrophysical variation due to the ellipsoidal variability \citep{Masuda2021}. 

\subsection{PHOEBE and ELC models of a giant + compact object binary}\label{section:phoebe}
We interpret the light curves as ellipsoidal variability and fit models to derive the orbital properties and dynamical masses of the red giant and its companion. Here we focus on the scenario where 2M0412 is a giant + compact object binary. We run additional models for the giant + star scenario in $\S$\ref{section:ccf}.

We initially fit the ZTF $r$-band and TESS light curves and the radial velocities phased with $P_{\rm orb}=81.2$~d using the differential evolution Markov Chain optimizer \citep{TerBraak2006} and the \verb"ELC" binary modelling code \citep{Orosz2000}. The optimizer was initialized using parameters estimated from the spectroscopic analysis and the Keplerian orbit fits from $\S$\ref{section:orbit}. The MCMC optimizer was run for 10,000 iterations using 21 chains. We fit for the mass, radius and temperature of the red giant ($M_{\rm giant}$, $R_{\rm giant}$, $T_{\rm eff, giant}$), the orbital inclination ($i$), the binary mass ratio ($q$), the observed radial velocity semi-amplitude ($K$), the systemic velocity ($v_\gamma$) and a nuisance parameter that accounts for errors in the phasing, assuming uniform priors. We included additional priors for the temperature ($T_{\rm eff, giant}=4150\pm100$~K), radius ($R_{\rm giant}=29\pm1~R_\odot$), surface gravity ($\log(g)=1.2\pm0.2$) and $v_{\rm rot} \, \textrm{sin} \, i=13.5\pm1.0~\rm km ~s^{-1}$. We also ran an additional set of models including the phased ZTF $g$-band light curve. 

From the \verb"ELC" posteriors, we obtain $M_{\rm giant}=0.988^{+0.022}_{-0.037}~M_\odot$, $M_{\rm comp}=4.673^{+0.123}_{-0.228}~M_\odot$, $T_{\rm eff, giant}=3870^{+13}_{-9}$~K, $R_{\rm giant}=35.7^{+0.2}_{-0.4}~R_\odot$, $i=35.47^{+1.00}_{-0.5}^\circ$, $q=M_{\rm giant}/M_{\rm comp}=0.249^{+0.034}_{-0.051}$ and $K=41.987^{+0.020}_{-0.020}~\rm km ~s^{-1}$. Notably, the temperature of the giant is somewhat cooler than the spectroscopic and SED estimates from $\S$\ref{section:giant}. The implied radius of the giant in the ELC fits ($R_{\rm giant}\simeq36~R_\odot$) is significantly larger than the SED estimate ($R_{\rm giant}\simeq29~R_\odot$). These results remain consistent if we also include the ZTF $g$-band light curve in the fits. The \verb"ELC" models also indicate that the red giant is almost filling its Roche lobe in a semi-detached orbital configuration.

%The \verb"ELC" models imply that the companion to 2M0412 is fairly massive with $M_{\rm comp}\simeq4.3-4.7~M_\odot$. 

Next, we simultaneously fit the ZTF $r$-band, and \textit{TESS} $T$-band light curves along with the radial velocities of the giant using \verb"PHOEBE" 2.3 \citep{Phoebe2016,Horvat2018,Conroy2020}. We assume that the companion to the red giant is a compact object and fix it to be a small ($R=3\times10^{-6}~R_\odot$), cold ($T_{\rm eff} =300$~K) black body, use the simplest and fastest eclipse model (\verb"eclipse_method=only_horizon"). We do not consider the effects of irradiation and reflection in our models. We adopt a logarithmic limb-darkening law and use coefficients from \citet{Claret2011} and \citet{Claret2017}. The parameters from the \verb"ELC" fits were used to initialize a MCMC sampler with 22 walkers, which was then run for 5000 iterations using the \verb"emcee" \citep{Foreman-Mackey2013} solver in \verb"PHOEBE" 2.3. 

Since our ELC models indicate that the giant is almost filling its Roche lobe, we initially constrained the orbital configuration in our \verb"PHOEBE" models to that of a semi-detached binary ($f=R_{\rm giant}/R_{\rm Roche, giant}=1$). We fit for the binary mass ratio $q=M_{\rm giant}/M_{\rm comp}$, orbital inclination ($i$), the semi-major axis of the red giant ($a_{\rm giant}\sin i$), the systemic velocity of the binary ($v_\gamma$) and the effective temperature of the giant ($T_{\rm eff, giant}$). We marginalize over the passband luminosities and nuisance parameters that account for underestimated errors in the light curves. We adopt Gaussian priors on the effective temperature ($T_{\rm eff, giant}=4200\pm100$~K), the radius ($R_{\rm giant}=29\pm1~R_\odot$), the inclination ($i=41\pm4^\circ$), the mass ratio ($q=0.25\pm0.05$) and the semi-major axis of the giant ($a_{\rm giant}\sin i=66\pm1~R_\odot$) based on the ELC fits and the analysis in $\S$\ref{section:giant}.  

From this fit, we obtain $P_{\rm orb}=81.16839^{+0.00044}_{-0.00045}~\rm d$, $a_{\rm giant}\sin i=67.103^{+0.029}_{-0.028}~R_{\odot}$, ${v_\gamma}=-47.316^{+0.011}_{-0.010}~\rm km~ s^{-1}$, $M_{\rm giant}=1.108^{+0.090}_{-0.101}~M_\odot$, $M_{\rm comp}=4.234^{+0.068}_{-0.075}~M_\odot$, $T_{\rm eff, giant}=4050^{+100}_{-110}$~K, $R_{\rm giant}=37.2^{+1.1}_{-1.1}~R_\odot$, $i=37.87^{+0.32}_{-0.36}^\circ$, and $q=M_{\rm giant}/M_{\rm comp}=0.261^{+0.019}_{-0.021}$. We also ran an additional set of models including the ZTF $g$-band light curve with consistent results. The results from the \verb"PHOEBE" models are consistent with those derived from the ELC models. The radius of the giant in the \verb"PHOEBE" models (${\sim}35-37~R_\odot$) is again significantly different from the SED radius (${\sim}29~R_\odot$). However, the definition of the radius in \verb"PHOEBE" differs from the definition of the photometric radius derived from the SED. \verb"PHOEBE" accounts for the non-spherical geometry in tidally distorted stars and reports an equivalent radius that is essentially the radius of a sphere containing the volume of the star. For red giant stars that fill their Roche lobes, the equivalent radius from \verb"PHOEBE" can be ${\lesssim}10\%$ larger than the photometric radius (e.g., \citealt{Miller2021}). While the different radius definitions may explain some of the difference between the \verb"PHOEBE" and SED radius estimates, it does not entirely account for the discrepancy in the radii.

Next, we fit \verb"PHOEBE" models to the ZTF $r$-band and TESS $T$-band light curves with the radius of the giant fixed to $R_{\rm giant}=23$, 25, 27, 29, 31 and $33~R_\odot$.  Here, we remove the semi-detached constraint and do not assume that the giant fills its Roche lobe. We assumed circular orbits at a period of $P_{\rm orb} =81.16839~ \rm d$ and kept the temperature of the giant fixed at $T_{\rm eff, giant}=4200~ \rm K$. We adopt the RV orbit from our initial \verb"PHOEBE" model and only fit for the mass ratio and inclination. These results are summarized in Table \ref{tab:phoebefitsrfixed}. The reported errors are purely statistical and do not consider systematic effects (veiling, etc.) in the derivation of the binary solution.

The mass of the giant increases monotonically and fairly rapidly with radius, $M_{\rm giant}\simeq0.35$, 0.43, 0.51, 0.60, 0.69, and $0.81~ M_\odot$, while the mass of the companion increases more slowly, $M_{\rm comp} \simeq 2.07$, 2.29, 2.58, 2.97, 3.28, and $3.59~M_\odot$. For $R_{\rm giant}=23~R_\odot$, the mass of the giant approaches the He core mass expected for a giant with $L_{\rm giant}\simeq230~L_\odot$, which is $M_{\rm core}\simeq0.34~M_\odot$ (Equation \ref{eq:coremass}). This implies that the radius of the giant must be $R_{\rm giant}\gtrsim23~R_\odot$. The mass ratio increases slowly, $q\simeq0.1699$, 0.1881, 0.1983, 0.1995, 0.2112, 0.2251 and the inclination drops rapidly with radius, $i=47.8$, 46.3, 44.4, 41.9, 40.6 and $39.5^\circ$. These models indicate that the giant is heavily stripped. With increasing radius, the Roche filling factor for the giant approaches unity. Therefore, we suspect that the significantly large radius estimate from the initial semi-detached models is a result of forcing the giant to completely fill its Roche lobe.


As our fiducial model for the remainder of the paper, we adopt the \verb"PHOEBE" model which matches the SED radius of $R_{\rm giant}\simeq29~R_\odot$. In this model, the companion mass is $M_{\rm comp}=2.972^{+0.017}_{-0.015}~M_\odot$, which implies a mass gap compact object if the companion is non-stellar. The mass of the giant is $M_{\rm comp}=0.595^{+0.002}_{-0.006}~M_\odot$ and the binary mass ratio is $q=M_{\rm giant}/M_{\rm comp}=0.1995^{+0.0010}_{-0.0010}$. The orbital inclination is $i_{\rm orb}=41.91^{+0.12}_{-0.10}^\circ$, consistent with the estimates from $v_{\rm rot} \, \textrm{sin} \, i$ ($\S$\ref{section:giant}). In this model, the giant nearly fills its Roche lobe with $f=R_{\rm giant}/R_{\rm Roche, giant}\simeq0.97$. This model is a good fit to the ZTF $r$-band, the \textit{TESS} $T$-band light curve, and the radial velocities (Figure \ref{lcs}). 

We can compare our estimates of the mass ratio to that obtained by the relation
\begin{equation}
    \label{eq:qrot}
    v_{\rm rot} \, \textrm{sin}~i/K_{\rm giant}=0.462~q^{1/3}(1+q)^{2/3} 
\end{equation} which assumes that the giant's rotation is synchronized with the binary orbit and that it completely fills its Roche lobe (see, for e.g., \citealt{Wade1988,Torres2002}). Using the HIRES measurement of $v_{\rm rot} \, \textrm{sin} \, i=13.3\pm1.0 \, \rm km \,s^{-1}$ and the RV semi-amplitude from the \verb"PHOEBE" models ($K_{\rm giant}$), we obtain $q=0.23\pm0.03,$ which is consistent with the mass ratio obtained in the \verb"PHOEBE" models (Table \ref{tab:phoebefitsrfixed}).

In summary, our \verb"PHOEBE" models indicate that the orbital inclination of 2M0412 is in the range $\sim39.5-47.8^\circ$ depending on the radius of the gaint. The companion to the red giant should be fairly massive with $M_{\rm comp}\simeq2.1-3.6~M_\odot$. Even if the companion is itself a binary of two stars, this mass estimate exceeds the 2 star SED limit in $\S$\ref{section:giant} ($M_{\rm binary}<2.6~M_\odot$) for radii $R_{\rm giant}\gtrsim27~R_\odot$. The inferred mass of the red giant ($M_{\rm giant}\simeq0.35-0.81~M_\odot$) is inconsistent with the single star MIST evolutionary tracks in $\S$\ref{section:giant} and instead imply that the giant is heavily stripped. In the absence of evidence for a stellar companion, the simplest explanation for the mass of the companion is that it is a non-interacting black hole in the ``mass-gap'' between $3-5~M_\odot$ \citep{Ozel2010,Farr2011}. We discuss other scenarios in $\S$\ref{section:darkcomp}. 



\begin{table*}
	\centering
	\caption{Summary of the orbital and component parameters from the PHOEBE models for a giant + compact object binary at fixed radii. We assumed a circular orbit with $P_{\rm orb} =81.16839~ \rm d$ and $a_{\rm giant}\sin i=67.103~R_{\odot}$  with the temperature of the giant fixed at to $T_{\rm eff, giant}=4200~ \rm K$. The reported errors are purely statistical and do not include systematic effects.}
	\label{tab:phoebefitsrfixed}
\begin{tabular}{rrrrrrr}
		\hline
	\vspace{2mm}		
		 Parameter & $R=23~R_\odot$ & $R=25~R_\odot$ & $R=27~R_\odot$ & $R=29~R_\odot$ & $R=31~R_\odot$ & $R=33~R_\odot$\\
	$d~(\rm kpc)$ & 3.2 & 3.5 & 3.8 & 4.1 & 4.4 & 4.7 \\		
		\hline
	\vspace{2mm}		
	$i_{\rm orb}~(^\circ)$  & $47.82^{+0.10}_{-0.10}$ & $46.34^{+0.14}_{-0.12}$ & $44.40^{+0.11}_{-0.11}$ & $41.91^{+0.12}_{-0.10}$ & $40.58^{+0.11}_{-0.10}$ & $39.51^{+0.11}_{-0.10}$\\	
	\vspace{2mm}
	$q_{\rm orb}$ & $0.1699^{+0.0010}_{-0.0011}$ & $0.1881^{+0.0011}_{-0.0011}$ & $0.1983^{+0.0009}_{-0.0008}$ & $0.1995^{+0.0010}_{-0.0010}$ & $0.2112^{+0.0009}_{-0.0009}$ & $0.2251^{+0.0008}_{-0.0008}$ \\
	\hline	
	\vspace{2mm}
	$f=R_{\rm giant}/R_{\rm Roche, giant}$ & 0.90 & $0.92$ & $0.94$ & $0.96$ & 0.97 & 0.98 \\		
	\hline	
	\vspace{2mm}	
	$M_{\rm giant}~(M_{\odot})$  & $0.351^{+0.038}_{-0.051}$ &  $0.432^{+0.003}_{-0.003}$ &  $0.511^{+0.002}_{-0.002}$ & $0.595^{+0.002}_{-0.006}$ & $0.693^{+0.002}_{-0.002}$ & $0.807^{+0.002}_{-0.002}$ \\
	$M_{\rm comp}~(M_{\odot})$  & $2.071^{+0.005}_{-0.011}$ &  $2.294^{+0.012}_{-0.013}$ &  $2.579^{+0.013}_{-0.013}$ & $2.972^{+0.017}_{-0.015}$ & $3.280^{+0.016}_{-0.019}$ & $3.586^{+0.012}_{-0.019}$ \\
	\hline
	\vspace{2mm}	
	$a_{\rm orb}$ $(R_{\odot})$  & $106.0^{+0.1}_{-0.2}$ & $110.2^{+0.2}_{-0.2}$ & $114.9^{+0.2}_{-0.2}$ & $120.5^{+0.2}_{-0.2}$ & $125.0^{+0.2}_{-0.2}$ & $129.2^{+0.2}_{-0.2}$\\
	\vspace{2mm}
	$a_{\rm comp}$ $(R_{\odot})$  & $15.4^{+0.1}_{-0.1}$ & $17.5^{+0.1}_{-0.1}$  & $19.0^{+0.1}_{-0.1}$ & $20.1^{+0.1}_{-0.1}$ & $21.8^{+0.1}_{-0.1}$ & $23.7^{+0.1}_{-0.1}$\\
	\vspace{2mm}
	$a_{\rm RG}$ $(R_{\odot})$  & $90.6^{+0.2}_{-0.2}$ & $92.8^{+0.2}_{-0.2}$ & $95.9^{+0.2}_{-0.2}$ & $100.5^{+0.2}_{-0.2}$ & $103.2^{+0.2}_{-0.2}$ & $105.5^{+0.2}_{-0.2}$\\		
\hline

\end{tabular}
\end{table*}



\begin{figure*}
	
	\includegraphics[width=0.7\textwidth]{phoebe_fits.pdf}
		\vspace{-0.2cm}	
    \caption{The normalized ZTF $g$, ZTF $r$ and TESS $T$-band light curves for 2M0412 as a function of orbital phase (defined with the epoch of maximal RV at $\phi=0.75$). The binned light curves for the ZTF $g$ and ZTF $r-$ band light curves are shown as black points. The scatter in the bins are shown as errorbars. The best-fitting giant + compact object binary models from PHOEBE are also shown.}
    \label{lcs}
\end{figure*}

\clearpage
\clearpage



\subsubsection{Comparison to single-star stellar models}

We use the spectroscopic parameters, 2MASS $JHK_s$ photometry and the EDR3 distance from \citet{Bailer-Jones2021} as priors to infer the physical properties of the giant using the MESA Isochrones and Stellar Tracks (MIST; \citealt{Dotter2016,Choi2016}) and \verb"isoclassify" \citep{Huber2017,Berger2020} to derive stellar parameters through isochrone fitting. As the best fit, we obtain $M_{\rm giant}=0.81^{+0.08}_{-0.04}~M_\odot$, $R_{\rm giant}=29.9^{+2.3}_{-2.1}~R_\odot$, $T_{\rm eff, giant}=4164\pm77$~K, $L_{\rm giant}= 244 ^{+38}_{-31}~ L_\odot$, $\log(g)=1.4\pm0.1$, and an estimated age ${\sim}15.5^{+3.0}_{-4.6}~{\rm Gyr}$. These results are inconsistent with the properties of the giant derived from the spectra and the SED. However, in $\S$\ref{section:phoebe} we discuss evidence that the giant is stripped and that the mass as inferred from single star tracks is over-estimated.

The surface gravity of the giant determined from the spectroscopic analysis and isochrone fitting is consistent with that inferred from the \verb"PHOEBE" models for the ellipsoidal variations presented in $\S$\ref{section:phoebe} ($\log(g)_{\rm PHOEBE}=1.19\pm0.01$). Given the spectroscopic $\log(g)$ and the radius of the giant from those models ($\S$\ref{section:phoebe}), the spectroscopic mass is $M_{\rm giant,spec}=0.9\pm0.6~M_\odot$, consistent with the mass of the giant derived from the \verb"PHOEBE" models. Based on the \citet{vanBelle1999} temperature scale for giants, our temperature estimates are consistent with a K4/K5 giant. The absolute $V$-band magnitude ($M_V\simeq-0.5\pm0.1$) is consistent with luminosity class III stars \citep{Straizys1981}. For single-star evolution, the spectroscopic measurement of $\log(g)$ suggests that the giant is currently evolving along the upper red giant branch (see Figure \ref{loggteff}). The giant is more luminous than the red clump, implying that it has not yet undergone a helium flash.
